Beyond Lorentzian Symmetry

This thesis presents a framework in which to explore kinematical symmetries beyond the standard Lorentzian case. This framework consists of an algebraic classification, a geometric classification, and a derivation of the geometric properties required to define physical theories on the classified spacetime geometries. The work completed in substantiating this framework for kinematical, super-kinematical, and super-Bargmann symmetries constitutes the body of this thesis. To this end, the classification of kinematical Lie algebras in spatial dimension $D = 3$, as presented in [3, 4], is reviewed; as is the classification of spatially-isotropic homogeneous spacetimes of [5]. The derivation of geometric properties such as the non-compactness of boosts, soldering forms and vielbeins, and the space of invariant affine connections is then presented. We move on to classify the $\mathcal{N}=1$ kinematical Lie superalgebras in three spatial dimensions, finding 43 isomorphism classes of Lie superalgebras. Once these algebras are determined, we classify the corresponding simply-connected homogeneous (4|4)-dimensional superspaces and show how the resulting 27 homogeneous superspaces may be related to one another via geometric limits. Finally, we turn our attention to generalised Bargmann superalgebras. In the present work, these will be the $\mathcal{N}=1$ and $\mathcal{N}=2$ super-extensions of the Bargmann and Newton-Hooke algebras, as well as the centrally-extended static kinematical Lie algebra, of which the former three all arise as deformations. Focussing solely on three spatial dimensions, we find $9$ isomorphism classes in the $\mathcal{N}=1$ case, and we identify $22$ branches of superalgebras in the $\mathcal{N}=2$ case.

==> Generalised_Bargmann_Spacetimes/GBAs/gba.tex <==
gba

==> Generalised_Bargmann_Spacetimes/GBSs/gbs.tex <==
\section{Classification of Klein pairs}
\label{sec:class-lie-pairs}

In this section we classify equivalence classes of Klein pairs $(\g,\h)$
where $\g$ is one of the Lie algebras in Table~\ref{tab:ce-summary}
and $\h \subset \g$ is a (pre-)admissible Lie subalgebra. For each
$\g$ in Table~\ref{tab:ce-summary} we determine, if necessary, the
automorphism group $\Aut\g$ and its action on the (pre-)admissible Lie
subalgebras.

\subsection{Klein pairs associated with Lie algebra \#1}
\label{sec:liep-assoc-1}

The automorphism group of the Lie algebra \#1 is the group of matrices
\begin{equation}
  \Aut\g = \left\{
    \begin{pmatrix}
      a & b & & \\ c & d & & \\ & & \lambda & \zero \\ & & \mu \Delta
      & \Delta
    \end{pmatrix} \middle | a,b,c,d,\lambda,\mu \in \RR, \Delta = ad -
  bc \neq 0, \lambda \neq 0\right\},
\end{equation}
acting on generators $(\B,\P,H,Z)$ as
\begin{equation}
  \B \mapsto a\B + c \P \qquad \P \mapsto b\B + d\P \qquad H \mapsto
  \lambda H + \mu \Delta Z \qquad\text{and}\qquad Z \mapsto \Delta Z.
\end{equation}
Any vectorial subspace $W_1 =\spn{\alpha \B + \beta \P}$ can
be brought to $\spn{\B}$ via an automorphism.  This means
that there is (up to equivalence) a unique pre-admissible subalgebra:
\begin{enumerate}[label=(B\arabic*)]
\item $\spn{\J,\B}$.
\end{enumerate}


Under an automorphism, a scalar subspace $W_0 = \spn{\sigma H +
  \tau Z}$ is sent to $\spn{\sigma \lambda H + (\sigma \mu
  + \tau) \Delta   Z}$.   If $\sigma = 0$, then $W_0 = \spn{Z}$, whereas if $\sigma \neq 0$, then by choosing $\mu$
appropriately, we can assume that $\tau = 0$ and hence $W_0 = \spn{Z}$.

In summary, we have two inequivalent admissible subalgebras:
\begin{enumerate}[label=(P\arabic*)]
\item $\spn{\J,\B, Z}$, and
\item $\spn{\J,\B, H}$.
\end{enumerate}

\subsection{Klein pairs associated with Lie algebra \#2}
\label{sec:liep-assoc-2}

The automorphism group has two connected components:
\begin{equation}
  \Aut \g = \left\{
    \begin{pmatrix}
      a & \zero & & \\ \zero & d & & \\ & & 1 & \zero \\ & & \mu \Delta  & \Delta
    \end{pmatrix} \middle | a,d,\mu \in \RR, \Delta = ad \neq
    0\right\} \bigcup
   \left\{
    \begin{pmatrix}
      \zero & b & & \\ c & \zero & & \\ & & -1 & \zero \\ & & \mu \Delta  & \Delta
    \end{pmatrix} \middle | b,c,\mu \in \RR, \Delta = -bc \neq  0\right\}.
\end{equation}
There are two orbits of $\Aut\g$ on the vectorial subspaces:
$\spn{\B}$ and $\spn{\B+\P}$, so that there are two pre-admissible
subalgebras:
\begin{enumerate}[label=(B\arabic*),start=2]
\item $\spn{\J,\B}$, and
\item $\spn{\J,\B+\P}$
\end{enumerate}

There are two orbits on the scalar subspaces: $\spn{H}$ and $\spn{Z}$.
In principle there are four cases to consider, however $W = \spn{\B+\P, H}$ does not give rise to
subalgebra.  Therefore there are three inequivalent admissible subalgebras:
\begin{enumerate}[label=(P\arabic*),start=3]
\item $\spn{\J,\B,Z}$,
\item $\spn{\J,\B,H}$, and
\item $\spn{\J,\B+\P,Z}$.
\end{enumerate}

\subsection{Klein pairs associated with Lie algebra \#3}
\label{sec:liep-assoc-3}

The automorphism group has again two connected components:
\begin{multline}
  \Aut \g = \left\{
    \begin{pmatrix}
      a & b & & \\ -b & a & & \\ & & 1 & \zero \\ & & \mu \Delta  & \Delta
    \end{pmatrix} \middle | a,b,\mu \in \RR, \Delta = a^2+b^2 \neq
    0\right\}\\ \bigcup
   \left\{
    \begin{pmatrix}
      a & b & & \\ b & -a & & \\ & & -1 & \zero \\ & & \mu \Delta  & \Delta
    \end{pmatrix} \middle | a,b,\mu \in \RR, \Delta = -a^2-b^2 \neq  0\right\}.
\end{multline}
We may always rotate the vectorial subspace so that $W_1 =
\spn{\B}$, so that there is a unique pre-admissible subalgebra:
\begin{enumerate}[label=(B\arabic*),start=4]
\item $\spn{\J,\B}$.
\end{enumerate}
There are two orbits of scalar subspaces: $\spn{H}$ and $\spn{Z}$, but
the former does not give rise to a subalgebra.  Therefore, there is a
unique admissible subalgebra for this Lie algebra:
\begin{enumerate}[label=(P\arabic*),start=6]
\item $\h= \spn{\J,\B,Z}$.
\end{enumerate}

\subsection{Klein pairs associated with Lie algebra \#4}
\label{sec:liep-assoc-4}

The automorphism group here is
\begin{equation}
  \Aut\g = \left\{
    \begin{pmatrix}
      a & \zero & & \\ c & \lambda a & & \\ & & \lambda & \zero \\ & & \mu \Delta
      & \Delta
    \end{pmatrix} \middle | a,c,\lambda,\mu \in \RR, \Delta = \lambda a^2 \neq 0\right\}.
\end{equation}
There are two orbits on vectorial subspaces $\spn{\B}$ and
$\spn{\P}$, so there are two inequivalent pre-admissible subalgebras:
\begin{enumerate}[label=(B\arabic*),start=5]
\item $\spn{\J,\B}$, and
\item $\spn{\J,\P}$.
\end{enumerate}
There are two orbits on scalar subspaces
$\spn{H}$ and $\spn{Z}$, but $\spn{\J,\B,H}$ is not a subalgebra.  Therefore there are
three inequivalent admissible subalgebras:
\begin{enumerate}[label=(P\arabic*),start=7]
\item $\h= \spn{\J,\B,Z}$,
\item $\h= \spn{\J,\P,Z}$, and
\item $\h= \spn{\J,\P,H}$.
\end{enumerate}

\subsection{Klein pairs associated with Lie algebra \#5}
\label{sec:liep-assoc-5}

Lie algebras \#5 -- \#7 in the table are trivial central extensions $\g =
\k \oplus \RR H$, where $\k$ is a kinematical Lie algebra but with
basis $\J,\B,\P,Z$.  Indeed, $\k = \so(D+1,1)$ in \#5, $\k = \so(D+2)$
(for $\varepsilon=1$) and $\so(D,2)$ (for $\varepsilon=-1$) in
\#6$_\varepsilon$ and $\k = \e$ (for $\varepsilon=1$) and $\k = \p$
(for $\varepsilon=-1$) in \#7$_\varepsilon$, where $\e$ and $\p$ are,
respectively, the euclidean and Poincaré Lie algebras.

The automorphism groups $\Aut\g$ and $\Aut\k$ are related as follows.
Let $\varphi \in \Aut\g$.  Then for all $X \in \k$,
\begin{equation}
  \varphi(X) = \psi(X) + \alpha(X) H \qquad\text{and}\qquad \varphi(H)
  = Y + \lambda H,
\end{equation}
for some $\psi : \k \to \k$, $\alpha \in \k^*$, $Y \in \k$ and
$\lambda \in \RR$.  Demanding that $\varphi$ be an automorphism, we
find that $\psi \in \Aut\k$, $\alpha \in [\k,\k]^o$, $Y \in \z(\k)$
and $\lambda\neq 0$.\footnote{Here $\z(\k)$ denotes the centre of $\k$
  and if $W \subset V$ are vector spaces, then $W^\circ \subset V^*$
  denotes the annihilator of $W$: those linear functions of $V$ which
  vanish on $W$.}  The Lie algebras \#5 and \#6$_\varepsilon$ are such
that $\k$ is simple, so that $[\k,\k] = \k$ and $\z(\k) = 0$. The Lie
algebras \#7$_\varepsilon$ are such that $\k$ is isomorphic to either
the euclidean or the Poincaré Lie algebra, and these too have $[\k,\k]
= \k$ and $\z(\k)= 0$.  Therefore for $\g$ one of the Lie algebras in
\#5 -- \#7, $\Aut\g \cong \Aut\k \times \RR^\times$.

The automorphisms for Lie algebra \#5 are given by
\begin{equation}
  \Aut \g = \left\{
    \begin{pmatrix}
      \sigma\cosh\theta & \sinh\theta & & \\
      \Delta\sinh\theta & \Delta\sigma\cosh\theta & & \\
      & & \Delta & \zero \\
      & & \zero & \lambda
    \end{pmatrix} \middle | \sigma,\Delta \in \{\pm1\}, \theta \in\RR,\lambda\in\RR^\times
  \right\} \cong O(1,1) \times \RR^\times.
\end{equation}
% \begin{equation}
%   \Aut \g = \left\{
%     \begin{pmatrix}
%       a & \zero & & \\ \zero & a^{-1} & & \\ & & 1 & \zero \\ & & \zero  & \lambda
%     \end{pmatrix} \middle | a,\lambda \in \RR^\times\right\} \bigcup
%    \left\{
%     \begin{pmatrix}
%       \zero & b & & \\ b^{-1} & \zero & & \\ & & -1 & \zero \\ & & \zero  & \lambda
%     \end{pmatrix} \middle | b,\lambda \in \RR^\times\right\}.
% \end{equation}

There are three choices of vectorial subspace for Lie algebra \#5 giving
rise to three inequivalent pre-admissible Lie subalgebras:
\begin{enumerate}[label=(B\arabic*),start=7]
\item $\spn{\J,\B+\P}$,
\item $\spn{\J,\P}$, and
\item $\spn{\J,\B}$.
\end{enumerate}
There are three possible scalar subspaces $\spn{Z}$, $\spn{H}$ or
$\spn{H+Z}$, but in all we have only five admissible subalgebras:
\begin{enumerate}[label=(P\arabic*),start=10]
\item $\spn{\J,\B+\P,H}$, 
\item $\spn{\J,\B+\P,Z}$,
\item $\spn{\J,\B+\P,H+Z}$,
\item $\spn{\J,\P,H}$, and
\item $\spn{\J,\B,H}$.
\end{enumerate}

\subsection{Klein pairs associated with Lie algebras \#6$_\varepsilon$}
\label{sec:liep-assoc-6}

In this case the automorphisms are given by
\begin{equation}
  \Aut \g = \left\{
    \begin{pmatrix}
      \cos\theta & -\sin\theta & & \\ \sin\theta & \cos\theta & & \\ & & \lambda & \zero \\ & & \zero  & 1
    \end{pmatrix} \middle | \theta \in \RR,~\lambda\in\RR^\times \right\} \bigcup
   \left\{
    \begin{pmatrix}
      \cos\theta & \sin\theta & & \\ \sin\theta & -\cos\theta & & \\ & & \lambda & \zero \\ & & \zero  & -1
    \end{pmatrix} \middle | \theta \in \RR,~\lambda \in \RR^\times\right\}.
\end{equation}
There is precisely one pre-admissible subalgebra up to equivalence:
\begin{enumerate}[label=(B\arabic*),start=10]
\item $\spn{\J,\B}$
\end{enumerate}
and precisely one admissible subalgebra up to equivalence:
\begin{enumerate}[label=(P\arabic*),start=15]
\item $\spn{\J,\B,H}$.
\end{enumerate}

\subsection{Klein pairs associated with Lie algebras \#7$_\varepsilon$}
\label{sec:liep-assoc-7}

The automorphisms here are
\begin{equation}
  \Aut\g = \left\{
    \begin{pmatrix}
      \pm 1 & \zero & & \\ c & \pm \lambda & & \\ & & \lambda & \zero
      \\ & &
      \zero & \mu
    \end{pmatrix} \middle | c,\lambda,\mu \in \RR, \lambda\mu \neq 0\right\}.
\end{equation}

There are two choices of vectorial subspaces up to the action of
$\Aut\g$ and hence two inequivalent pre-admissible subalgebras:
\begin{enumerate}[label=(B\arabic*),start=11]
\item $\spn{\J,\B}$, and
\item $\spn{\J,\P}$.
\end{enumerate}
In the former case, the only scalar subspace leading to an admissible
subalgebra is $\spn{H}$, whereas in the latter we have three:
$\spn{Z}$, $\spn{H}$ and $\spn{H+Z}$.  This gives a total of four
admissible subalgebras up to equivalence:
\begin{enumerate}[label=(P\arabic*),start=16]
\item $\spn{\J,\B,H}$,
\item $\spn{\J,\P,Z}$,
\item $\spn{\J,\P,H}$, and
\item $\spn{\J,\P,H+Z}$.
\end{enumerate}

\subsection{Klein pairs associated with Lie algebra \#8}
\label{sec:liep-assoc-8}

The automorphisms here are
\begin{equation}
  \Aut\g =  \left\{
    \begin{pmatrix}
      a & b & & \\ c & d & & \\ & & 1 & \zero \\ & & \mu & \Delta
    \end{pmatrix} \middle | a,b,c,d,\mu \in \RR, \Delta = ad -bc \neq 0\right\}.
\end{equation}
Using automorphisms, we may bring the vectorial subspace to $W_1 =
\spn{\B}$, so there is up to equivalence a unique pre-admissible
subalgebra:
\begin{enumerate}[label=(B\arabic*),start=13]
\item $\spn{\J,\B}$.
\end{enumerate}

There are two possibilities for the scalar subspace: $\spn{Z}$ and
$\spn{H}$.  This gives rise to two admissible subalgebras up to
equivalence:
\begin{enumerate}[label=(P\arabic*),start=20]
\item $\spn{\J,\B,Z}$, and
\item $\spn{\J,\B,H}$.
\end{enumerate}

\subsection{Klein pairs associated with Lie algebra \#9$_\gamma$}
\label{sec:liep-assoc-9}

The automorphism group here is
\begin{equation}
  \Aut\g =  \left\{
    \begin{pmatrix}
      a & \zero & & \\ \zero & d & & \\ & & 1 & \zero \\ & & \mu & ad
    \end{pmatrix} \middle | a,d,\mu \in \RR, ad \neq 0\right\}.
\end{equation}
There are three possible vectorial subspaces leading to pre-admissible
subalgebras:
\begin{enumerate}[label=(B\arabic*),start=14]
\item $\spn{\J,\B}$,
\item $\spn{\J,\P}$, and
\item $\spn{\J,\B+\P}$.
\end{enumerate}
For each such vectorial subspaces, we can take the scalar subspace to
be either $\spn{Z}$ or $\spn{H}$, except that $\spn{\J,\B+\P,H}$ is
not a subalgebra.  In total there are five admissible subalgebras:
\begin{enumerate}[label=(P\arabic*),start=22]
\item $\spn{\J,\B,Z}$, 
\item $\spn{\J,\B,H}$, 
\item $\spn{\J,\P,Z}$,
\item $\spn{\J,\P,H}$, and
\item $\spn{\J,\B+\P,Z}$.
\end{enumerate}

\subsection{Klein pairs associated with Lie algebra \#10}
\label{sec:liep-assoc-10}

The automorphism group here is
\begin{equation}
  \Aut\g =  \left\{
    \begin{pmatrix}
      a & b & & \\ \zero & a & & \\ & & 1 & \zero \\ & & \mu & a^2
    \end{pmatrix} \middle | a,b,\mu \in \RR, a \neq 0\right\}.
\end{equation}
There are up to the action of $\Aut\g$ two pre-admissible subalgebras:
\begin{enumerate}[label=(B\arabic*),start=17]
\item $\spn{\J,\B}$, and
\item $\spn{\J,\P}$.
\end{enumerate}
There are also two admissible scalar subspaces $\spn{Z}$ or
$\spn{H}$.  However $\spn{\J,\P,H}$ is not a subalgebra, so that there
are only three inequivalent admissible subalgebras:
\begin{enumerate}[label=(P\arabic*),start=27]
\item $\spn{\J,\B,Z}$, 
\item $\spn{\J,\B,H}$, and
\item $\spn{\J,\P,Z}$.
\end{enumerate}

\subsection{Klein pairs associated with Lie algebra \#11$_\chi$}
\label{sec:liep-assoc-11}

Here the automorphism group is
\begin{equation}
  \Aut\g =  \left\{
    \begin{pmatrix}
      a & b & & \\ -b & a & & \\ & & 1 & \zero \\ & & \mu & \Delta
    \end{pmatrix} \middle | a,b,\mu \in \RR, \Delta = a^2 + b^2 \neq 0\right\}.
\end{equation}
Under the action of the automorphisms, we can
bring any vectorial subspace to $W_1 = \spn{\B}$, so there is only one
pre-admissible subalgebra up to equivalence:
\begin{enumerate}[label=(B\arabic*),start=19]
\item $\spn{\J,\B}$.
\end{enumerate}
There is only one scalar subspace leading to a subalgebra: $W_0 =
\spn{Z}$, so there is a unique admissible subalgebra up to
equivalence:
\begin{enumerate}[label=(P\arabic*),start=30]
\item $\spn{\J,\B,Z}$.
\end{enumerate}

\subsection{Klein pairs associated with Lie algebras \#12$_\varepsilon$}
\label{sec:liep-assoc-12}

The automorphisms here are
\begin{equation}
  \Aut\g =  \left\{
    \begin{pmatrix}
      a & \zero & & \\ - a \mu \varepsilon & d & & \\ & & 1 & \zero \\ & & \mu & a d
    \end{pmatrix} \middle | d,\mu \in \RR,\ a = \pm1,\ d \neq 0\right\}.
\end{equation}
There are, up to equivalence, two pre-admissible subalgebras:
\begin{enumerate}[label=(B\arabic*),start=20]
\item $\spn{\J,\B}$, and
\item $\spn{\J,\P}$.  
\end{enumerate}
There are two possible scalar subspaces: $\spn{Z}$ and $\spn{H}$,
but $\spn{\J,\B,Z}$ is not a subalgebra.  Therefore there are, up to
equivalence, three admissible Lie subalgebras:
\begin{enumerate}[label=(P\arabic*),start=31]
\item $\spn{\J,\B,H}$,
\item $\spn{\J,\P,Z}$, and
\item $\spn{\J,\P,H}$.
\end{enumerate}

\subsection{Summary of results}
\label{sec:summary-results}

Table~\ref{tab:hbs-summary} summarises the equivalence classes of Klein
pairs for homogeneous Bargmann spaces which we classified above.  Each
row in the table is one such Klein pair with sequential label ``B\#''.
The label ``L\#'' is the Lie algebra in Table~\ref{tab:ce-summary}.
The Lie brackets are expressed in a basis where the pre-admissible
subalgebra is $\spn{\J,\B}$.

Table~\ref{tab:gbs-summary} summarises the above classification of
Klein pairs for homogeneous spacetimes.  Each row in the table is one
Klein pair with sequential label ``P\#''.  The label ``L\#'' is the Lie
algebra in Table~\ref{tab:ce-summary} and the label ``B\#'' is the
associated homogeneous Bargmann space in Table~\ref{tab:hbs-summary}.
The Lie brackets are expressed in a basis where the admissible
subalgebra $\h = \spn{\J,\B,Z}$.  In some cases we have made
additional changes of basis consistent with these requirements to
uniformise the notation.

\begin{table}[h!]
  \centering
  \caption{Klein pairs for ($D+2$)-dimensional homogeneous Bargmann spaces ($D\geq 3$)}
  \label{tab:hbs-summary}
  \rowcolors{2}{blue!10}{white}
  \resizebox{\textwidth}{!}{
  \begin{tabular}{*{2}{l|}*{5}{>{$}l<{$}}|l}
   \multicolumn{1}{c|}{B\#} & \multicolumn{1}{c|}{L\#} & \multicolumn{5}{c|}{Nonzero Lie brackets in addition to $[\J,\J] = \J$, $[\J, \B] = \B$, $[\J,\P] = \P$}& \multicolumn{1}{c}{Comments} \\\toprule
    1 & 1 & [\B,\P] = Z & & & & & \\
    2 & 2 & [\B,\P] = Z & [H,\B] = \B & [H,\P] = - \P & & &\\
    3 & 2 & [\B,\P] = Z & [H,\B] = \P & [H,\P] = \B & & &\\
    4 & 3 & [\B,\P] = Z & [H,\B] = \P & [H,\P] = -\B & & &\\
    5 & 4 & [\B,\P] = Z & [H,\B] = \P & & & &\\
    6 & 4 & [\B,\P] = Z & & [H,\P] = -\B & & &\\
    7 & 5 & [\B,\P] = Z + \J & [Z,\B] = \B & [Z,\P] = - \P & & &\\
    8 & 5 & [\B,\P] = Z & [Z,\B] = -\P & [Z,\P] = -\B & [\B,\B]=\J & [\P,\P] = - \J & \\
    9 & 5 & [\B,\P] = Z & [Z,\B] = \P & [Z,\P] = \B & [\B,\B]= -\J & [\P,\P] = \J & \\
    10$_\varepsilon$ & 6$_\varepsilon$ & [\B,\P] = Z & [Z,\B] = -\varepsilon \P & [Z,\P] = \varepsilon \B & [\B,\B] = \varepsilon \J & [\P,\P] = \varepsilon \J & $\varepsilon= \pm 1$\\
    11$_\varepsilon$ & 7$_\varepsilon$ & [\B,\P] = Z & [Z,\B] = -\varepsilon \P & & [\B,\B] = \varepsilon \J & & $\varepsilon= \pm 1$\\
    12$_\varepsilon$ & 7$_\varepsilon$ & [\B,\P] = Z & & [Z,\P] = \varepsilon \B & & [\P,\P] = \varepsilon \J & $\varepsilon= \pm 1$\\
    13 & 8 & [\B,\P] = Z & [H,\B] = \B & [H,\P] = \P & [H,Z] = 2 Z & & \\
    14$_\gamma$ & 9$_\gamma$ & [\B,\P] = Z & [H,\B] = \gamma \B & [H,\P] = \P & [H,Z] = (1+\gamma)Z & & $-1<\gamma<1$\\
    15$_\gamma$ & 9$_\gamma$ & [\B,\P] = Z & [H,\B] = \B & [H,\P] = \gamma \P & [H,Z] = (1+\gamma)Z & & $-1<\gamma<1$\\
    16$_\gamma$ & 9$_\gamma$ & [\B,\P] = Z & [H,\B] = \P & [H,\P] = -\gamma \B + (1+\gamma)\P & [H,Z] = (1+\gamma)Z & & $-1<\gamma<1$\\
    17 & 10 & [\B,\P] = Z & [H,\B] = \B & [H,\P] = \B + \P & [H,Z] = 2 Z & & \\
    18 & 10 & [\B,\P] = Z & [H,\B] = \P & [H,\P] = -\B + 2 \P & [H,Z] = 2 Z & & \\
    19$_\chi$ & 11$_\chi$ & [\B,\P] = Z & [H,\B] = \P & [H,\P] = -(1+\chi^2) \B + 2 \chi \P & [H,Z] = 2 \chi Z & & $\chi>0$ \\
    20$_\varepsilon$ & 12$_\varepsilon$ & [\B,\P] = Z & [Z,\B] = \varepsilon \P & [H,\P] = \P & [H,Z] = Z & [\B,\B] = - \varepsilon \J & $\varepsilon=\pm1$\\
    21$_\varepsilon$ & 12$_\varepsilon$ & [\B,\P] = Z & [H,\B] = \B & [Z,\P] = -\varepsilon\B & [H,Z] = Z & [\P,\P] = -\varepsilon \J & $\varepsilon=\pm1$ \\\bottomrule
  \end{tabular}}
\end{table}

\begin{table}[h!]
  \centering
  \caption{Klein pairs for ($D+1$)-dimensional Bargmann spacetimes ($D\geq 3$)}
  \label{tab:gbs-summary}
  \rowcolors{2}{blue!10}{white}
  \resizebox{\textwidth}{!}{
  \begin{tabular}{*{3}{l|}*{5}{>{$}l<{$}}|l}
   \multicolumn{1}{c|}{P\#} & \multicolumn{1}{c|}{B\#} & \multicolumn{1}{c|}{L\#} & \multicolumn{5}{c|}{Nonzero Lie brackets in addition to $[\J,\J] = \J$, $[\J, \B] = \B$, $[\J,\P] = \P$}& \multicolumn{1}{c}{Comments} \\\toprule
    1 & 1 & 1 & [\B,\P] = Z & & & & & \\
    2 & 1 & 1 & [\B,\P] = H & & & & & \\
    3 & 2 & 2 & [\B,\P] = Z & [H,\B] = \B & [H,\P] = - \P & & &\\
    4 & 2 & 2 & [\B,\P] = H & [Z,\B] = \B & [Z,\P] = - \P & & &\\
    5 & 3 & 2 & [\B,\P] = Z & [H,\B] = \P & [H,\P] = \B & & &\\
    6 & 4 & 3 & [\B,\P] = Z & [H,\B] = \P & [H,\P] = -\B & & &\\
    7 & 5 & 4 & [\B,\P] = Z & [H,\B] = -\P & & & &\\
    8 & 6 & 4 & [\B,\P] = Z & & [H,\P] = -\B & & &\\
    9 & 6 & 4 & [\B,\P] = H & & [Z,\P] = \B & & &\\
    10 & 7 & 5 & [\B,\P] = H + \J & [H,\B] = \B & [H,\P] = - \P & & &\\
    11 & 7 & 5 & [\B,\P] = Z + \J & [Z,\B] = \B & [Z,\P] = - \P & & & \\
    12 & 7 & 5 & [\B,\P] = Z - H + \J & [Z,\B] = \B & [Z,\P] = - \P & & & \\
    13 & 8 & 5 & [\B,\P] = H & [H,\B] = -\P & [H,\P] = -\B & [\B,\B]=\J & [\P,\P] = - \J & \\
    14 & 9 & 5 & [\B,\P] = H & [H,\B] = \P & [H,\P] = \B & [\B,\B]= -\J & [\P,\P] = \J & \\
    15$_\varepsilon$ & 10$_\varepsilon$ & 6$_\varepsilon$ & [\B,\P] = H & [H,\B] = -\varepsilon \P & [H,\P] = \varepsilon \B & [\B,\B] = \varepsilon \J & [\P,\P] = \varepsilon \J & $\varepsilon= \pm 1$\\
    16$_\varepsilon$ & 11$_\varepsilon$ & 7$_\varepsilon$ & [\B,\P] = H & [H,\B] = -\varepsilon \P & & [\B,\B] = \varepsilon \J & & $\varepsilon= \pm 1$\\
    17$_\varepsilon$ & 12$_\varepsilon$ & 7$_\varepsilon$ & [\B,\P] = Z & & [Z,\P] = \varepsilon \B & & [\P,\P] = \varepsilon \J & $\varepsilon= \pm 1$\\
    18$_\varepsilon$ & 12$_\varepsilon$ & 7$_\varepsilon$ & [\B,\P] = H & & [H,\P] = \varepsilon \B & & [\P,\P] = \varepsilon \J & $\varepsilon= \pm 1$\\
    19$_\varepsilon$ & 12$_\varepsilon$ & 7$_\varepsilon$ & [\B,\P] = H & [H,\P] = \varepsilon \B  & [Z,\P] = \varepsilon \B & & [\P,\P] = \varepsilon \J & $\varepsilon= \pm 1$\\
    20 & 13 & 8 & [\B,\P] = Z & [H,\B] = \B & [H,\P] = \P & [H,Z] = 2 Z & & \\
    21 & 13 & 8 & [\B,\P] = H & [Z,\B] = \B & [Z,\P] = \P & [Z,H] = 2 H & & \\
    22$_\gamma$ & 14$_\gamma$ & 9$_\gamma$ & [\B,\P] = Z & [H,\B] = \gamma \B & [H,\P] = \P & [H,Z] = (1+\gamma)Z & & $-1<\gamma<1$\\
    23$_\gamma$ & 14$_\gamma$ & 9$_\gamma$ & [\B,\P] = H & [Z,\B] = \gamma \B & [Z,\P] = \P & [Z,H] = (1+\gamma)H & & $-1<\gamma<1$\\
    24$_\gamma$ & 15$_\gamma$ & 9$_\gamma$ & [\B,\P] = Z & [H,\B] = \B & [H,\P] = \gamma \P & [H,Z] = (1+\gamma)Z & & $-1<\gamma<1$\\
    25$_\gamma$ & 15$_\gamma$ & 9$_\gamma$ & [\B,\P] = H & [Z,\B] = \B & [Z,\P] = \gamma \P & [Z,H] = (1+\gamma)H & & $-1<\gamma<1$\\
    26$_\gamma$ & 16$_\gamma$ & 9$_\gamma$ & [\B,\P] = Z & [H,\B] = \P & [H,\P] = -\gamma \B + (1+\gamma)\P & [H,Z] = (1+\gamma)Z & & $-1<\gamma<1$\\
    27 & 17 & 10 & [\B,\P] = Z & [H,\B] = \B & [H,\P] = \B + \P & [H,Z] = 2 Z & & \\
    28 & 17 & 10 & [\B,\P] = H & [Z,\B] = \B & [Z,\P] = \B + \P & [Z,H] = 2 H & & \\
    29 & 18 & 10 & [\B,\P] = Z & [H,\B] = \P & [H,\P] = - B + 2 \P & [H,Z] = 2 Z & & \\
    30$_\chi$ & 19$_\chi$ & 11$_\chi$ & [\B,\P] = Z & [H,\B] = \P & [H,\P] = -(1+\chi^2) \B + 2 \chi \P & [H,Z] = 2 \chi Z & & $\chi>0$ \\
    31$_\varepsilon$ & 20$_\varepsilon$ & 12$_\varepsilon$ & [\B,\P] = H & [H,\B] = \varepsilon \P & [Z,\P] = \P & [Z,H] = H & [\B,\B] = -\varepsilon \J & $\varepsilon=\pm1$ \\
    32$_\varepsilon$ & 21$_\varepsilon$ & 12$_\varepsilon$ & [\B,\P] = Z & [H,\B] = \B & [Z,\P] = -\varepsilon\B & [H,Z] = Z & [\P,\P] = -\varepsilon \J & $\varepsilon=\pm1$ \\
    33$_\varepsilon$ & 21$_\varepsilon$ & 12$_\varepsilon$ & [\B,\P] = H & [Z,\B] = \B & [H,\P] = -\varepsilon\B & [Z,H] = H & [\P,\P] = -\varepsilon \J & $\varepsilon=\pm1$\\\bottomrule
  \end{tabular}}
\end{table}

\section{Classification of spacetimes}
\label{sec:class-spac}

Having classified equivalence classes of Klein pairs we now refine the
classification by selecting only those which are effective and
geometrically realisable, since these are the ones which are in
one-to-one correspondence with simply-connected homogeneous Bargmann
spaces and spacetimes.

Let $\g$ be a generalised Bargmann algebra.  Recall that $\g$ has a
semisimple (since $D\geq 3$) Lie subalgebra $\r \cong \so(D)$.  This
imposes strong constraints on the nature of ideals contained in a
(pre-)admissible subalgebra $\h$.

If $\h$ is pre-admissible, the only possible ideal is the ideal $\b$
spanned by the boosts.  By inspection of the $[\B,\P]$ brackets for
the Klein pairs in Table~\ref{tab:hbs-summary}, we see that this is
never the case.  Therefore every such Klein pair is effective.

If $\h$ is now an admissible Lie subalgebra of $\g$, then there are
three kinds of possible ideals, of which only two\footnote{There is no
  case where the ideal is only the span of the $\{B_a\}$, since by
  construction $\g$ is a deformations of the centrally extended static
  Lie algebra and hence the Lie bracket $[\B,\P]$ always contains a
  nonzero scalar.} appear:
\begin{enumerate}
\item the ideal spanned by $Z$, or
\item the ideal spanned by the $\{B_a\}$ and $Z$.
\end{enumerate}
In the first case, quotienting by the ideal spanned by $Z$ gives a Klein
pair corresponding to a homogeneous kinematical spacetime; whereas in the second
case, quotienting by the ideal spanned by the $\{B_a\}$ and $Z$, gives
a Klein pair corresponding to a homogeneous aristotelian spacetime.
Homogeneous kinematical and aristotelian spacetimes were classified in
\cite{Figueroa-OFarrill:2018ilb} and further studied in \cite{Figueroa-OFarrill:2019sex}.

Referring to the numbers in Table~\ref{tab:gbs-summary}, we see that
Klein pairs P\#1,3,8 and \#24$_0$ correspond to the aristotelian static
spacetime, which is A\#21 in \cite{Figueroa-OFarrill:2018ilb}.  Similarly, Klein
pairs P\#20, 22$_\gamma$, 24$_{\gamma\neq 0}$ and 27 correspond to the
aristotelian spacetime denoted by A\#22 in \cite{Figueroa-OFarrill:2018ilb}.
Finally, Klein pairs 18$_\varepsilon$ and 32$_\varepsilon$ correspond to
the aristotelian spacetime with label A\#23$_\varepsilon$ in
\cite{Figueroa-OFarrill:2018ilb}.  This is summarised in the first of the three
sub-tables in Table~\ref{tab:gbs-kinematical}.  The other two
sub-tables in Table~\ref{tab:gbs-kinematical} list those non-effective
Klein pairs in Table~\ref{tab:gbs-summary} which correspond to
kinematical spacetimes, together with the label in
\cite{Figueroa-OFarrill:2018ilb} and, if known, the name.

\begin{table}[h!]
  \centering
  \caption{Klein pairs for ($D+1$)-dimensional aristotelian and kinematical spacetimes ($D\geq 3$)}
  \label{tab:gbs-kinematical}
  \begin{tabular}{l|l|l}
   \multicolumn{1}{c|}{P\#} & \multicolumn{1}{c|}{\cite{Figueroa-OFarrill:2018ilb}A\#} & \multicolumn{1}{c}{Name} \\\toprule
    1 & 21 & $\zS$ \\
    3 & 21 & $\zS$ \\
    8 & 21 & $\zS$ \\
    17$_\varepsilon$ & 23$_\varepsilon$ & \\
    20 & 22 & $\zTS$ \\
    22$_\gamma$ & 22 & $\zTS$ \\
    24$_{\gamma=0}$ & 21 & $\zS$ \\
    24$_{\gamma\neq 0}$ & 22 & $\zTS$ \\
    27 & 22 & $\zTS$ \\
    32$_\varepsilon$ & 23$_\varepsilon$ & \\\bottomrule
  \end{tabular}
  \qquad\qquad
  \begin{tabular}{l|l|l}
   \multicolumn{1}{c|}{P\#} & \multicolumn{1}{c|}{\cite{Figueroa-OFarrill:2018ilb}S\#} & \multicolumn{1}{c}{Name} \\\toprule
    2 & 13 & $\zC$ \\
    5 & 8 & $\zdSG$ \\
    6 & 10 & $\zAdSG$\\
    7 & 7 & $\zG$\\
    10 & 16 & $\znrC$\\
    13 & 2 & $\zdS$ \\
    14 & 6 & $\HH$ \\
    15$_{+1}$ & 3 & $\zAdS$\\\bottomrule
  \end{tabular}
  \qquad\qquad
  \begin{tabular}{l|l|l}
   \multicolumn{1}{c|}{P\#} & \multicolumn{1}{c|}{\cite{Figueroa-OFarrill:2018ilb}S\#} & \multicolumn{1}{c}{Name} \\\toprule
    15$_{-1}$ & 5 & $\SS$ \\
    16$_{+1}$ & 1 & $\MM$\\
    16$_{-1}$ & 4 & $\EE$ \\
    18$_{+1}$ & 15 & $\zAdSC$\\
    18$_{-1}$ & 14 & $\zdSC$ \\
    26$_\gamma$ & 9$_\gamma$ & $\ztdSG_{\gamma \in (-1,1)}$\\
    29 & 9$_1$ & $\ztdSG_1$ \\
    30$_\chi$ & 11$_\chi$ & $\ztAdSG_{\chi>0}$\\\bottomrule
  \end{tabular}
\end{table}

This then leaves a list of effective Klein pairs which are studied in
more detail in the next section. These Klein pairs are
P\#4, 9, 11, 12, 19$_\varepsilon$, 21, 23$_\gamma$, 25$_\gamma$, 28, 31$_\varepsilon$ and
33$_\varepsilon$.  We find it convenient to extract them from
Table~\ref{tab:gbs-summary} and place them in
Table~\ref{tab:gbs-effective-lie-pairs}.  We notice that many of the
generalised Bargmann Lie algebras in
Table~\ref{tab:gbs-effective-lie-pairs} are $\ZZ$-graded with $Z$
playing the rôle of the grading element.  The only cases where this
fails are P\#9, 19$_\varepsilon$ and 28, where $\ad_Z$ is not
diagonalisable.

\begin{table}[h!]
  \centering
  \caption{Effective Klein pairs for ($D+1$)-dimensional Bargmann spacetimes ($D\geq 3$)}
  \label{tab:gbs-effective-lie-pairs}
  \rowcolors{2}{blue!10}{white}
  \resizebox{\textwidth}{!}{
  \begin{tabular}{*{3}{l|}*{5}{>{$}l<{$}}|l}
   \multicolumn{1}{c|}{P\#} & \multicolumn{1}{c|}{B\#} & \multicolumn{1}{c|}{L\#} & \multicolumn{5}{c|}{Nonzero Lie brackets in addition to $[\J,\J] = \J$, $[\J, \B] = \B$, $[\J,\P] = \P$}& \multicolumn{1}{c}{Comments} \\\toprule
    4 & 2 & 2 & [\B,\P] = H & [Z,\B] = \B & [Z,\P] = - \P & & &\\
    9 & 6 & 4 & [\B,\P] = H & & [Z,\P] = \B & & &\\
    11 & 7 & 5 & [\B,\P] = Z + \J & [Z,\B] = \B & [Z,\P] = - \P & & & \\
    12 & 7 & 5 & [\B,\P] = Z - H + \J & [Z,\B] = \B & [Z,\P] = - \P & & & \\
    19$_\varepsilon$ & 12$_\varepsilon$ & 7$_\varepsilon$ & [\B,\P] = H & [H,\P] = \varepsilon \B & [Z,\P] = \varepsilon \B & & [\P,\P] = \varepsilon \J & $\varepsilon= \pm 1$\\
    21 & 13 & 8 & [\B,\P] = H & [Z,\B] = \B & [Z,\P] = \P & [Z,H] = 2 H & & \\
    23$_\gamma$ & 14$_\gamma$ & 9$_\gamma$ & [\B,\P] = H & [Z,\B] = \gamma \B & [Z,\P] = \P & [Z,H] = (1+\gamma)H & & $-1<\gamma<1$\\
    25$_\gamma$ & 15$_\gamma$ & 9$_\gamma$ & [\B,\P] = H & [Z,\B] = \B & [Z,\P] = \gamma \P & [Z,H] = (1+\gamma)H & & $-1<\gamma<1$\\
    28 & 17 & 10 & [\B,\P] = H & [Z,\B] = \B & [Z,\P] = \B + \P & [Z,H] = 2 H & & \\
    31$_\varepsilon$ & 20$_\varepsilon$ & 12$_\varepsilon$ & [\B,\P] = H & [H,\B] = \varepsilon \P & [Z,\P] = \P & [Z,H] = H & [\B,\B] = -\varepsilon \J & $\varepsilon=\pm1$ \\
    33$_\varepsilon$ & 21$_\varepsilon$ & 12$_\varepsilon$ & [\B,\P] = H & [Z,\B] = \B & [H,\P] = -\varepsilon\B & [Z,H] = H & [\P,\P] = -\varepsilon \J & $\varepsilon=\pm1$\\\bottomrule
  \end{tabular}}
\end{table}

\subsection{Geometric Realisability}

Having identified the effective Klein pairs for $(D+2)$-dimensional Bargmann spaces
and the $(D+1)$-dimensional Bargmann spacetimes, we can now ask which of the 
pairs are geometrically realisable.  Recall, a Klein pair $(\g, \h)$ is said to be
geometrically realisable if there exists a Lie group $\Ggr$ with Lie algebra $\g$
such that the unique connected Lie subgroup $\Hgr$ corresponding to the
subalgebra $\h$ is closed.  Demonstrating this property requires different
techniques depending on whether we are in the homogeneous Bargmann space 
case or the Bargmann spacetime case; therefore, this section is divided into
two.  We will first consider the effective Klein pairs for homogeneous
Bargmann spaces before tackling the effective Klein pairs for the Bargmann
spacetimes.  It will be shown that all effective Klein pairs are also
geometrically realisable in both instances.

\subsubsection{Homogeneous Bargmann spaces}

In the case of homogeneous Bargmann spaces, we have $\h = \spn{\J,\B}$, as
in the kinematical instances of \cite{Figueroa-OFarrill:2019sex}.  Here, we will use
this fact along with the following observation to prove that each of the effective
Klein pairs in Table \ref{tab:hbs-summary} is geometrically realisable.

Let $\g$ be one of the algebras in Table \ref{tab:hbs-summary}, and $\g' = [\g, \g]$
be its first derived ideal.  We notice that, in all cases, $\g'$ is a kinematical algebra.
The exact mapping is given in Table \ref{tab:gbs-ideals}.  In particular, we always have
that $(\g', \h)$ is a geometrically realisable Klein pair.  Therefore, we want to use
this information to show that $(\g, \h)$ is also geometrically realisable.

Begin by letting $\tilde{\Ggr}$ be the unique simply-connected Lie group whose
Lie algebra is $\g$.  We want to show that $\Hgr \subset \tilde{\Ggr}$, with Lie
algebra $\h \subset \g$, is closed. We know that since $(\g', \h)$ is geometrically
realisable, $\Hgr \subset \tilde{\Ggr'}$ is closed.  In addition,  the derived subgroup
$\Ggr'$, with Lie algebra $\g'$, is closed and connected in $\tilde{\Ggr}$.  Our
strategy now runs as follows.  If we can show that the covering map $p: \tilde{\Ggr'}
\rightarrow \Ggr'$ is closed, then $\Hgr$ will be a closed subgroup in $\Ggr'$.
With $\Hgr \subset \Ggr'$ closed and $\Ggr' \subset \tilde{\Ggr}$ also closed,
we will have that $\Hgr$ is closed in $\tilde{\Ggr}$, as desired. 

To show that $p: \tilde{\Ggr'} \rightarrow \Ggr'$ is closed, we use the following
important points.
\begin{enumerate}
	\item A covering map $p: \tilde{\Ggr'} \rightarrow \Ggr'$ is closed if it is finite, and 
	\item for $\tilde{\Ggr'}$ simply connected and $\Ggr'$ connected, $\ker\, p \cong \pi_1(\Ggr')$.
\end{enumerate}
Therefore, if we can show that $\pi_1(\Ggr')$ is finite, we will have lifted the
geometric realisability of $(\g', \h)$ to $(\g, \h)$.  The $\Ggr'$ associated
with each of the homogeneous Bargmann spaces are listed in Table
\ref{tab:gbs-ideals}, where $\ISO(p, q) = \SO(p, q) \ltimes \mathbb{R}^{p, q}$,
and $\IISO(p) = (\SO(p) \ltimes \mathbb{R}^{p}) \ltimes \mathbb{R}^{p+1}$
for all $p, q \in \mathbb{N}$.  It is known that $\pi_1(\SO(p, q)) = \pi_1(\SO(p)) \times
\pi_1(\SO(q))$, and that $\SO(n) = \mathbb{Z}_2$ for $n \geq 3$.  In addition,
$\pi_1(\SO(1))$ is trivial.  Therefore, $\SO(D+1, 1)$ and $\SO(D)$ have finite
fundamental groups, such that B\# 7, 8, 9, and 10$_{-1}$ are all geometrically
realisable.  Note, we cannot use this result for B\#10$_{+1}$, as $\pi_1(\SO(2))
 = \mathbb{Z}$.  We will return to this case at the end of the section. 

We can now extend our results to the ``inhomogeneous" cases, $\ISO(p, q)$ and $\IISO(p, q)$.
Since $\ISO(p, q)$ is a semi-direct product, we may write the following short exact sequence
\begin{equation}
	0 \rightarrow \mathbb{R}^{p, q} \rightarrow \ISO(p, q) \rightarrow \SO(p, q) \rightarrow 0.
\end{equation}
Applying the homotopy functor, we have
\begin{equation}
	\ldots \rightarrow \pi_1(\mathbb{R}^{p, q}) \rightarrow \pi_1(\ISO(p, q)) \rightarrow
	\pi_1(\SO(p, q)) \rightarrow \pi_0(\mathbb{R}^{p, q}) \rightarrow \ldots .
\end{equation}
Since $\pi_0(\mathbb{R}^{p, q}) = \pi_1(\mathbb{R}^{p, q}) = 0$, the above sequence reduces to 
\begin{equation}
	0 \rightarrow \pi_1(\ISO(p, q)) \rightarrow
	\pi_1(\SO(p, q)) \rightarrow 0 .
\end{equation}
Thus, $\pi_1(\ISO(p, q)) \cong \pi_1(\SO(p, q))$.  This result tells us that $\pi_1(\ISO(D)) =
\pi_1(\ISO(D+1)) = \pi_1(\ISO(D, 1)) = \mathbb{Z}_2$ for $D \geq 3$.  Applying the same
argument again, $\pi_1(\ISO(D)) = \mathbb{Z}_2$ tells us that $\pi_1(\IISO(D)) = \mathbb{Z}_2$.
These results demonstrate the geometric realisability of all the other Klein pairs in
Table \ref{tab:hbs-summary} except B\#10$_{+1}$, which we shall consider now.

The Lie algebra $\g$, in this instance, takes the
form $\g = \g' \oplus \mathbb{R}$, where $\mathbb{R}$ is trivial central extension of 
$\g' = \so(D, 2)$.  As with all the previous cases, we know that $(\g', \h)$ is a geometrically
realisable Klein pair and we want to extend this property to $(\g, \h) = (\g' \oplus \mathbb{R}, \h)$.
Because we have a direct sum of Lie algebras, we can integrate $\g$ to $\tilde{\Ggr'} \times
\mathbb{R}$ with the product topology.  We know that $\Hgr \subset \tilde{\Ggr'}$ is closed;
therefore, embedding $\Hgr$ into $\tilde{\Ggr'} \times \mathbb{R}$ with $\Hgr \rightarrow
\Hgr \times \{0\}$, we have that $\Hgr \cong \Hgr \times \{0\} \subset \tilde{\Ggr'} \times
\mathbb{R}$ is closed.  Thus, $(\g, \h)$ is geometrically realisable. 


\begin{table}[h!]
  \centering
  \caption{Derived ideals of Klein pairs for homogeneous Bargmann spaces}
  \label{tab:gbs-ideals}
  \begin{tabular}{l|l|l|l}
   \multicolumn{1}{c|}{B\#} & \multicolumn{1}{c|}{\cite{Figueroa-OFarrill:2018ilb}S\#} & \multicolumn{1}{c|}{Name} & \multicolumn{1}{c}{$\Ggr'$} \\\toprule
    1 & 13 & $\zC$ & $\IISO(D)$ \\
    2 & 13 & $\zC$ & $\IISO(D)$ \\
    3 & 13 & $\zC$ & $\IISO(D)$ \\
    4 & 13 & $\zC$ & $\IISO(D)$ \\
    5 & 13 & $\zC$ & $\IISO(D)$ \\
    6 & 13 & $\zC$ & $\IISO(D)$ \\
    7 & 16 & $\zLC$ & $\SO(D+1, 1)$ \\
    8 & 2 & $\zdS$ & $\SO(D+1, 1)$\\
    9 & 6 & $\HH$ & $\SO(D+1, 1)$ \\
    10$_{+1}$ & 3 & $\zAdS$ & $\SO(D, 2)$ \\
    10$_{-1}$ & 5 & $\SS$ & $\SO(D)$ \\
    11$_{+1}$ & 1 & $\MM$ & $\ISO(D, 1)$ \\
    11$_{-1}$ & 4 & $\EE$ & $\ISO(D)$ \\\bottomrule
  \end{tabular}
   \qquad\qquad
  \begin{tabular}{l|l|l|l}
   \multicolumn{1}{c|}{B\#} & \multicolumn{1}{c|}{\cite{Figueroa-OFarrill:2018ilb}S\#} & \multicolumn{1}{c|}{Name} & \multicolumn{1}{c}{$\Ggr'$} \\\toprule
   12$_{+1}$ & 15 & $\zAdSC$ & $\ISO(D, 1)$ \\
    12$_{-1}$ & 14 & $\zdSC$ & $\ISO(D+1)$ \\
    13 & 13 & $\zC$ & $\IISO(D)$  \\
    14$_\gamma$ & 13 & $\zC$ & $\IISO(D)$ \\
    15$_\gamma$ & 13 & $\zC$ & $\IISO(D)$  \\
    16$_\gamma$ & 13 & $\zC$ & $\IISO(D)$\\
    17 & 13 & $\zC$ & $\IISO(D)$ \\
    18 & 13 & $\zC$ & $\IISO(D)$\\
    19$_\chi$ & 13 & $\zC$ & $\IISO(D)$ \\
    20$_{+1}$ & 4 & $\EE$ & $\ISO(D)$  \\
    20$_{-1}$ & 1 & $\MM$ & $\ISO(D, 1)$\\
    21$_{+1}$ & 14 & $\zdSC$ & $\ISO(D+1)$ \\
    21$_{-1}$ & 15 &  $\zAdSC$ & $\ISO(D, 1)$ \\\bottomrule
  \end{tabular}
  \caption*{In each table, the first column indicates the B\# identifier for the Klein pair $\g$ and the second column states
  the S\# for the derived ideal $\g'$.  The third column names the spacetime associated with the derived ideal, and,
  finally, the last column gives the Lie group $\Ggr'$ corresponding to the Lie algebra $\g'$.}
\end{table}

\subsubsection{Bargmann spacetimes}

We now turn to the Klein pairs highlighted in Table \ref{tab:gbs-effective-lie-pairs},
which describe the $(D+1)$-dimensional Bargmann spacetimes.  In
these instances, we have $\h = \spn{\J, \B, Z}$.  To begin, we notice that each
Lie algebra $\g$, except P\#11 and 12, may be written
as a semi-direct product of the derived ideal $\g' = [\g, \g]$ and the abelian
subalgebra $\a = \spn{Z}$, $\g = \a \ltimes \g'$.  Additionally, each derived
ideal has an associated kinematical spacetime.  For the mapping, see Table
\ref{tab:gbs-ideals}.  Letting $\b = \spn{\J, \B}$, such that $\h = \a \ltimes \b$,
the geometrically realisable Klein pair contained in $\g$ is then $(\g', \b)$.
Our aim, for now, is to extend the geometric realisability of $(\g', \b)$ to 
$(\g, \h) = (\a \ltimes \g', \a \ltimes \b)$.  We will come back to P\#11 and 12
later on. 

The key point in extending the geometric realisability is that
for any semi-direct product Lie algebra $\g = \a \ltimes \g'$, we can always
define a semi-direct product of simply-connected Lie groups $\tilde{\Ggr} =
\tilde{\Agr} \ltimes \tilde{\Ggr'}$, where the action of $\a$ on $\g'$ is
the differential of the  $\tilde{\Agr}$-action on $\tilde{\Ggr'}$ \cite{onishchik2012lie}.
Given that $\Bgr \subset \tilde{\Ggr}$ is closed, we then have that
$\tilde{\Agr} \ltimes \Bgr$ is closed in $\tilde{\Agr} \ltimes \tilde{\Ggr'}$.
This result shows the geometric realisablility of all the Bargmann spacetimes,
except for P\#11 and 12.

To demonstrate the geometric realisability of P\#11, we begin by noticing that
the brackets given in Table \ref{tab:gbs-effective-lie-pairs} are the
same as those for the Carrollian light-cone, $\zLC$ \cite{Figueroa-OFarrill:2018ilb}.  However,
there are two key difference between these cases.  The first difference is that P\#11
has a trivial central extension: $\g = \g' \oplus \mathbb{R}$, where $\g'
= [\g, \g]$ is isomorphic to the Lie algebra of $\zLC$. The second difference is that we want
the admissible Lie subalgebra $\h$ to contain $Z$, which is acting as
our time translation generator in $\g'$.  

We can now make use of the correspondence between P\#11 and
$\zLC$ in the following way.  Let $\b = \spn{\J, \B}$, such that the
geometrically realisable Klein pair associated with $\zLC$ in $\g$
is $(\g', \b)$.  We want to extend this property to $(\g',
\b \rtimes \a)$, where $\a = \spn{Z}$.  Once we have that $(\g',
\b \rtimes \a)$ is geometrically realisable,  it is not much work to
show that $(\g, \h) = (\g' \oplus \mathbb{R}, \b \rtimes \a)$ also
has this property.  In particular, we can use the same reasoning as
was used in the case of B\#10$_{+1}$.

The fact that we are able to extend the geometric realisability of
$(\g', \b)$ to $(\g', \b \rtimes \a)$ is very particular to this case.  We
notice that $\zLC^{D+1}$ has the topology $\mathbb{R} \times \SS^D$,
where the factor of $\mathbb{R}$ corresponds to our ``time" direction;
in this instance, the span of $Z$.  Therefore, by adding $Z$ to $\b$,
we take the quotient of $\zLC^{D+1}$ by its factor of $\mathbb{R}$,
leaving $\SS^D$ as the geometry associated with $(\g', \b \rtimes \a)$.
As in the case of B\#10$_{+1}$, the addition of the trivial central
extension to $\g'$ only adds a copy of $\mathbb{R}$ to the geometry;
therefore, P\#11 is geometrically realisable with topology $\SS^D \times
\mathbb{R}$.


\FIXMER{Now do P\#12.}  


\begin{table}[h!]
  \centering
  \caption{Derived ideals of Klein pairs for Bargmann spacetimes}
  \label{tab:gbs-ideals}
  \begin{tabular}{l|l|l|l}
   \multicolumn{1}{c|}{P\#} & \multicolumn{1}{c|}{\cite{Figueroa-OFarrill:2018ilb}S\#} & \multicolumn{1}{c|}{Name} \\\toprule
    4 & 13 & $\zC$  \\
    9 & 13 & $\zC$  \\
    19$_{+1}$ & 15 & $\zAdSC$  \\
    19$_{-1}$ & 14 & $\zdSC$ \\
    21 & 13 & $\zC$  \\
    23$_{\gamma}$ & 13 & $\zC$ \\\bottomrule
  \end{tabular}
   \qquad\qquad
  \begin{tabular}{l|l|l|l}
   \multicolumn{1}{c|}{P\#} & \multicolumn{1}{c|}{\cite{Figueroa-OFarrill:2018ilb}S\#} & \multicolumn{1}{c|}{Name} \\\toprule
    25$_\gamma$ & 13 & $\zC$  \\
    28 & 13 & $\zC$ \\
    31$_{+1}$ & 4 & $\EE$   \\
    31$_{-1}$ & 1 & $\MM$ \\
    33$_{+1}$ & 14 & $\zdSC$  \\
    33$_{-1}$ & 15 & $\zAdSC$  \\\bottomrule
  \end{tabular}
  \caption*{In each table, the first column indicates the P\# identifier for the Klein pair $\g$, the second column states
  the S\# for the derived ideal $\g'$, and the final column names the spacetime associated with the derived ideal.}
\end{table}

\begin{comment}

How about geometric realisability?  Recall that a Klein pair $(\g,\h)$
is geometrically realisable if the connected subgroup $\Hgr$ generated by
$\h$ in the simply-connected Lie group $\Ggr$ with Lie algebra $\g$ is
closed.  As discussed in \cite{Figueroa-OFarrill:2018ilb}, there a
several algebraic criteria which guarantee that this is the case.

One of them says that if the subalgebra $\h$ of a linear Lie algebra
$\g$ is its own normaliser, then the connected subgroup $\Hgr \subset
\Ggr$ to which it exponentiates is closed (see, e.g.,
\cite[Pr.~2.7.4]{MR1889121}) and $\Ggr/\Hgr$ is a geometric
realisation of $(\g,\h)$.  Ado's theorem (see, e.g.,
\cite[Ch.~VI]{MR559927})) guarantees that every generalised Bargmann
Lie algebra $\g$ is linear.  Inspection of the Lie algebras in
Table~\ref{tab:gbs-effective-lie-pairs} shows that $\h =
\spn{\J,\B,Z}$ is its own normaliser in all but the first 5 rows:
P4, P9, P11, P12 and P19$_\varepsilon$.  \FIXMEJ{How about them?}

\FIXMEJ{Geometric realisability of Bargmann spaces?}

\FIXMEJ{We had missed two Klein pairs which are effective: P\#9 and
  19$_\varepsilon$.  So things change from here on down.}
  
\end{comment}



==> Generalised_Bargmann_Spacetimes/GPs/gps.tex <==
In this section we analyse some geometric properties of the
homogeneous spaces associated to the effective Klein pairs in Tables
\ref{tab:hbs-summary} and \ref{tab:gbs-effective-lie-pairs}. Indeed,
to each such Klein pair $(\g,\h)$ there is associated (up lo local
isomorphism) a homogeneous space $\Ggr/\Hgr$, on which the group
$\Ggr$ with Lie algebra $\g$ acts transitively with generic stabiliser
the subgroup $\Hgr$ with Lie algebra $\h$. Many local geometrical
properties of a homogenous space $\Ggr/\Hgr$ can be deduced by
studying the infinitesimal description $(\g,\h)$.

We say that a pair $(\g,\h)$ is \textbf{reductive}, if there is a
vector space isomorphism $\g = \h \oplus \m$ such that $[\h,\m]
\subset \m$.  In addition, if $[\m,\m] \subset \h$, we say that
$(\g,\h)$ is \textbf{symmetric}.  If $(\g,\h)$ is reductive and
$[\m,\m] = 0$, then we say that it is \textbf{affine}.  This is not to
be confused with the notion of an ``affine symmetric space'' in
\cite{MR1393941}.  The rationale for calling such Klein pairs ``affine''
is that if such a Klein pair is effective and geometrically realisable,
then its unique simply-connected geometric realisation is an affine
space.

Even if $(\g,\h)$ is not reductive, there is a linear representation
of $\h$ on the quotient $\g/\h$, by virtue of $\h$ being a
subalgebra. This is called the \textbf{linear isotropy representation}
of $\h$.  There is a one-to-one correspondence between
$\Ggr$-invariant tensor fields on $\Ggr/\Hgr$ and $\Hgr$-invariant
tensors of the linear isotropy representation.  If we assume that
$\Ggr$ and $\Hgr$ are connected, then $\Hgr$-invariant tensors agree
with $\h$-invariant tensors.  It is therefore convenient to study in
detail the action of $\h$ on $\g/\h$.

Tables~\ref{tab:hbs-geoprops} and \ref{tab:gbs-geoprops} summarise the
geometrical properties of the ($D+2$)-dimensional homogeneous Bargmann
spaces and the ($D+1$)-dimensional homogeneous Bargmann spacetimes we
have classified.  A $\checkmark$ on the ``R''
column indicates that the Klein pair $(\g,\h)$ is reductive.  If
reductive, we can then ask whether it is symmetric and, if so, affine.
Again we use $\checkmark$ to indicate  the presence of those properties for the Klein pair on the
respective columns: ``S'' and ``A''.   The ``Invariants'' column lists
the $\h$-invariants in the representations $\g/\h$, $S^2(\g/\h)$ and
their duals.  We explain below how to calculate them.  Finally, the
column ``Comments'' contains any additional comments and/or an
identification of the relevant homogeneous space.

Let us explain the notation in the ``Invariants'' column. Our choice
of basis for $\g$ is such that a pre-admissible subalgebra is spanned
by $\J$ and $\B$, and an admissible subalgebra is spanned by $\J$,
$\B$ and $Z$.  This means that the linear isotropy representation in a
($D+2$)-dimensional homogeneous Bargmann space acts on the space
$\g/\h$ spanned by $\Pbar := \P \mod \h$, $\Hbar := H\mod \h$ and
$\Zbar := Z \mod \h$, where $\h$ is the pre-admissible subalgebra.  We
let $\pi^a$, $\eta$ and $\zeta$ denote the canonical dual basis for
$(\g/\h)^*$. In other words, they satisfy $\eta(\Hbar) = 1$, $\eta(\overline{P}_a) =
\eta(\Zbar) = 0$, $\pi^a(\overline{P}_b) = \delta^a_b$, $\pi^a(\Hbar)
= \pi^a(\Zbar) = 0$ and $\zeta(\Zbar) = 1$ and $\zeta(\Hbar) =
\zeta(\overline{P}_a) = 0$.

We are particularly interested in whether there are any
$\h$-invariants in the representations $\g/\h$, $S^2(\g/\h)$,
$(\g/\h)^*$ and $S^2(\g/\h)^*$.  Now, invariance under $\h$ implies,
in particular, invariance under the rotational subalgebra $\r$.  It is
easy to write down the possible rotational invariant tensors and
therefore we need only check invariance under $\B$.  The
action of $\B$ is induced by duality from the action on $\g/\h$ which
is given by
\begin{equation}
  B_a \cdot \Hbar = \overline{[B_a,H]}, \qquad
  B_a \cdot \Zbar = \overline{[B_a,Z]} \qquad\text{and}\qquad
  B_a \cdot \overline{P}_b = \overline{[B_a, P_b]},
\end{equation}
with the brackets being those of $\g$.  In practice, we can determine
this from Table~\ref{tab:hbs-summary}, by computing the brackets in
$\g$ and simply dropping any $\B$ or $\J$ from the right-hand side.

The only possible invariants in $\g/\h$ are proportional to $\Hbar$ and
$\Zbar$, which are invariant provided that $[\B,H] \in \h$ and
$[\B,Z] \in \h$, respectively.  Dually, the only possible
invariants in $(\g/\h)^*$ are proportional to $\eta$ and $\zeta$, which
are invariant provided that there is no $X \in \g$ such that $H$
(respectively, $Z$) appears in $[\B,X]$. The only rotational
invariants in $S^2(\g/\h)$ are linear combinations of $H^2$, $Z^2$,
$HZ$ and $P^2 := \delta^{ab} P_a P_b$, whereas in $S^2(\g/\h)^*$ are
$\eta^2$, $\zeta^2$, $\eta\zeta$ and $\pi^2 = \delta_{ab}\pi^a\pi^b$.

In the case of the $(D+1)$-dimensional homogeneous Bargmann
spacetimes, the story is very similar, except that now $Z$ is part of
the admissible subalgebra $\h = \spn{\J, \B, Z}$.  This means that we
must also check invariance under $Z$.

\begin{table}[h!]
  \centering
  \caption{Geometrical properties of ($D+2$)-dimensional homogeneous Bargmann spaces}
  \label{tab:hbs-geoprops}
  \rowcolors{2}{blue!10}{white}
  \begin{tabular}{l|l|*{4}{>{$}c<{$}|}l}
   \multicolumn{1}{c|}{B\#} & \multicolumn{1}{c|}{L\#} & \multicolumn{1}{c|}{R} & \multicolumn{1}{c|}{S} & \multicolumn{1}{c|}{A} & \multicolumn{1}{c|}{Invariants} & \multicolumn{1}{c}{Comments} \\\toprule
    1 & 1 & \checkmark & \checkmark & \checkmark  &  \eta, \pi^2, Z, H & \\
    2 & 2 & &  &  & \eta, \pi^2, Z, H & \\
    3 & 2 & \checkmark & \checkmark  &  & \eta, Z & \\
    4 & 3 & \checkmark & \checkmark  &  & \eta, Z & \\
    5 & 4 & \checkmark & \checkmark & \checkmark & \eta, Z & \\
    6 & 4 & \checkmark & \checkmark &   & \eta, \pi^2, Z, H & \\
    7 & 5 &  &  &  & \zeta, \pi^2, Z, H & \\
    8 & 5 & \checkmark & \checkmark &   & \zeta, \pi^2 - \eta^2, Z & \\
    9 & 5 & \checkmark & \checkmark &   & \zeta, \pi^2 + \eta^2, Z & \\
    10$_\varepsilon$ & 6$_\varepsilon$ & \checkmark & \checkmark &   & \zeta, \pi^2 + \varepsilon\eta^2, Z & $\varepsilon=\pm 1$ \\
    11$_\varepsilon$ & 7$_\varepsilon$ & \checkmark & \checkmark & \checkmark & \varepsilon \eta^2 + \varepsilon \pi^2 & $\varepsilon=\pm 1$ \\
    12$_\varepsilon$ & 7$_\varepsilon$ & \checkmark &  & & \zeta, \pi^2, Z, H & $\varepsilon=\pm 1$ \\
    13 & 8 &  & & & \eta, \pi^2, Z, H & \\
    14$_0$ & 9$_0$ & \checkmark &  & & \eta, \pi^2, Z, H & \\    
    14$_{\gamma\neq0}$ & 9$_{\gamma\neq0}$ &  & & & \eta, \pi^2, Z, H & $\gamma \in (-1,0)\cup(0,1)$ \\
    15$_\gamma$ & 9$_\gamma$ &  & & & \eta, \pi^2, Z, H & $\gamma \in (-1,1)$ \\
    16$_\gamma$ & 9$_\gamma$ & \checkmark &  & & \eta, \tfrac12 \pi^2 + \zeta \eta, Z & $\gamma \in (-1,1)$ \\
    17 & 10 &  & & & \eta, \pi^2, Z, H & \\
    18 & 10 & \checkmark &  & & \eta, \tfrac12 \pi^2 + \zeta \eta, Z & \\
    19$_\chi$ & 11$_\chi$ & \checkmark &  & & \eta, \tfrac12 \pi^2 + \zeta \eta, Z & $\chi > 0$ \\
    20$_\varepsilon$ & 12$_\varepsilon$ & \checkmark &  & & \eta, H, \pi^2 + \varepsilon \zeta^2 & $\varepsilon=\pm 1$ \\
    21$_\varepsilon$ & 12$_\varepsilon$ &  & & & \eta, \pi^2, Z, H & $\varepsilon=\pm 1$ \\\bottomrule
  \end{tabular}
\end{table}

\begin{table}[h!]
  \centering
  \caption{Geometrical properties of ($D+1$)-dimensional Bargmann spacetimes}
  \label{tab:gbs-geoprops}
  \rowcolors{2}{blue!10}{white}
  \begin{tabular}{l|l|l|*{4}{>{$}c<{$}|}l}
  \multicolumn{1}{c|}{P\#} & \multicolumn{1}{c|}{B\#} & \multicolumn{1}{c|}{L\#} & \multicolumn{1}{c|}{R} & \multicolumn{1}{c|}{S} & \multicolumn{1}{c|}{A} & \multicolumn{1}{c|}{Invariants} & \multicolumn{1}{c}{Comments} \\\toprule
    4 & 2 & 2 & \checkmark & \checkmark & \checkmark & H & \\
    9 & 6 & 4 &  &  &  &  H, \pi^2& \\
    11 & 7 & 5 &  &  &  &  H & \\
    12 & 7 & 5 &  & & & H & \\
    19$_\varepsilon$ & 12$_\varepsilon$ & 7$_\varepsilon$ &  & & & H, \pi^2 & \\
    21 & 13 & 8 & \checkmark & \checkmark & \checkmark & & \\
    23$_\gamma$ & 14$_\gamma$ & 9$_\gamma$ & \checkmark & \checkmark & \checkmark & &  $\gamma \in (-1,1)$\\
    25$_0$ & 15$_0$ & 9$_0$ & \checkmark & \checkmark & \checkmark & \pi^2 &  \\
    25$_{\gamma\neq0}$ & 15$_{\gamma\neq0}$ & 9$_{\gamma\neq0}$ & \checkmark & \checkmark & \checkmark & & $\gamma \in (-1,0)\cup(0,1)$ \\    
    28 & 17 & 10 &  & & & & \\
  31$_\varepsilon$ & 20$_\varepsilon$ & 12$_\varepsilon$ & \checkmark & \checkmark & \checkmark & & $\varepsilon=\pm 1$\\
  33$_\varepsilon$ & 21$_\varepsilon$ & 12$_\varepsilon$ & \checkmark & \checkmark &  & \pi^2 &  $\varepsilon=\pm 1$\\\bottomrule
  \end{tabular}
\end{table}

\FIXMEJ{In many cases in Table \ref{tab:gbs-geoprops}, the absence of
  invariants is due to $Z$ acting like a grading element.  This
  suggests perhaps looking at projective invariants; e.g., conformal
  classes of inner products,...}

\section{Further geometrical properties of homogeneous Bargmann
  spacetimes}
\label{sec:furth-geom-prop}

In this section we concentrate on the homogeneous spacetimes in
Table~\ref{tab:gbs-effective-lie-pairs} and discuss further
geometrical properties: fundamental vector fields, soldering form,
vielbein and invariant connections, following the methodology
explained in \cite{Figueroa-OFarrill:2019sex} for the kinematical spacetimes.

For each effective Klein pair $(\g,\h)$ in
Table~\ref{tab:gbs-effective-lie-pairs}, with $\h = \spn{\J,\B,Z}$, we
introduce exponential coordinates $(t,\x)$ such that $\sigma(t,\x) =
\exp(t H + \x \cdot \P)$ defines an analytic map from a neighbourhood
of $\boldsymbol{0} \in \RR^{D+1}$ to a neighbourhood of the identity
in $\Ggr$, which projects down to a neighbourhood of the identity
coset in the homogeneous space $M = \Ggr/\Hgr$.  We work out the
expression for the fundamental vector fields $\xi_X$ for $X \in \g$
relative to the exponential coordinates as well as the expression for
the soldering one-form and, in the reductive cases, also for the
connection one-form of the canonical invariant connection.  We also
invert the soldering form to find the vielbein.  Finally, we determine
the possible invariant affine connections.

The methodology is explained in \cite{Figueroa-OFarrill:2019sex}, but let us
record some of the relevant formulae.  Let $A = t H + \x \cdot \P$
and let us introduce the following analytic functions related to the
derivative of the exponential map:
\begin{equation}
  \begin{split}
    D(z) &= \frac{1-e^{-z}}{z} = 1 - \frac{z}2 + O(z^2)\\
    F(z) &= \frac{1}{D(z)} = 1 + \frac{z}2 + O(z^2)\\
    G(z) &= e^{-z} F(z) = 1 - \frac{z}2 + O(z^2).
  \end{split}
\end{equation}
The fundamental vector field $\xi_X$ for $X \in \g$ takes the form
\begin{equation}
  \xi_X = \tau \frac{\d}{\d t} + y^a \frac{\d}{\d x^a},
\end{equation}
where $(\tau, \y)$ are found by solving
\begin{equation}
  \tau H + \y \cdot \P = G(\ad_A) X - F(\ad_A) Y,
\end{equation}
for some $Y \in \h$.  In all cases, the fundamental vector field
generating the action of the rotations has the following standard
form:
\begin{equation}
  \xi_{J_{ab}} = x^b \frac{\d}{\d x^a} - x^a \frac{\d}{\d x^b}.
\end{equation}
Therefore it is only necessary to work out the expressions for
$\xi_H$, $\xi_Z$, $\xi_{B_a}$ and $\xi_{P_a}$.  A simple check of our
calculations is that the map $X \mapsto \xi_X$ is a Lie algebra
\emph{antihomomorphism}.

The soldering form $\theta$ is obtained by
projecting to $\g/\h$ the pull-back $\sigma^*\vartheta$ of the
left-invariant Maurer--Cartan one-form $\vartheta$ on $\Ggr$.  In the
reductive case, where $\g = \h \oplus \m$, then $\sigma^*\vartheta =
\theta + \omega$, where $\theta$ is the $\m$-component and $\omega$,
the $\h$-component, is the connection one-form for the canonical
invariant connection.  In any case, we can find $\theta$ (and, if
relevant, also $\omega$) by solving
\begin{equation}
  \sigma^*\vartheta = D(\ad_A) (dt H + d\x \cdot \P).
\end{equation}

Invariant connections are defined by $\h$-invariant linear maps
$\Lambda : \g \to \gl(\g/\h)$ with the normalisation condition that
$\left.\Lambda\right|_\h = \lambda$, the linear isotropy
representation.  In the reductive case, with $\g = \h \oplus \m$,
$\Lambda$ is determined, for all $X,Y \in \m$, by
\begin{equation}
  \Lambda_XY := \alpha(X,Y),
\end{equation}
where the $\h$-invariant bilinear map $\alpha : \m \times \m \to \m$
is called the Nomizu map of the invariant connection.  In the
reductive case there is a canonical invariant connection defined with
vanishing Nomizu map.  In the non-reductive case, it may well be the
case that there are no invariant connections.  If $\Lambda$ is an
invariant affine connection, its torsion and curvature are given by
\begin{equation}
  T(X,Y) = \Lambda_X Y - \Lambda_Y X - [X,Y] \mod \h
\end{equation}
and
\begin{equation}
  R(X,Y)Z = \Lambda_X\Lambda_Y Z - \Lambda_Y\Lambda_X Y -
  \Lambda_{[X,Y]} Z \mod \h.
\end{equation}
It follows from the invariance condition and the fact that we project
to $\g/\h$, that only the class of $X,Y,Z \in \g$ modulo $\h$
contributes to the above formulae, so that the torsion defines an
$\h$-invariant skew-symmetric bilinear map $T : \g/\h \times \g/\h \to
\g/\h$ and, similarly, the curvature defines an $\h$-invariant
skew-symmetric bilinear map $R : \g/\h \times \g/\h \to
\gl(\g/\h)$.  In the reductive case, we can take $X,Y,Z \in \m$ and
then the torsion and curvature of an invariant connection with Nomizu
map $\alpha$ are given by
\begin{equation}
  T(X,Y) = \alpha(X,Y) - \alpha(Y,X) - [X,Y]_{\m}
\end{equation}
and
\begin{equation}
  R(X,Y)Z = \alpha(X,\alpha(Y,Z)) - \alpha(Y,\alpha(X,Z)) -
  \alpha([X,Y]_{\m},Z) - \lambda_{[X,Y]_\h} Z.
\end{equation}

In the rest of this section we record the results of our calculations.

\subsection{Homogeneous spacetime P\#4}
\label{sec:homog-spac-p4}

With $A = t H + \x \cdot \P$ we find
\begin{equation}
  \ad_A H = 0 \qquad \ad_A Z = \x \cdot \P \qquad \ad_A \P = 0
  \qquad\text{and}\qquad \ad_A \B = - \x H,
\end{equation}
so that $\ad_A^2 = 0$.  Solving for the fundamental vector fields, we
find
\begin{equation}
  \xi_{H} = \frac{\d}{\d t} \qquad \xi_{P_a} = \frac{\d}{\d x^a}
  \qquad \xi_{B_a} = x^a \frac{\d}{\d t} \qquad\text{and}\qquad \xi_Z
  = - x^a \frac{\d}{\d x^a}.
\end{equation}
One checks that $[\xi_Z,\xi_{B_a}] = - \xi_{B_a}$, $[\xi_Z,\xi_{P_a}]
= \xi_{P_a}$ and that $[\xi_{B_a}, \xi_{P_b}] = - \delta_{ab} \xi_H$,
as expected.

The soldering form is given by
\begin{equation}
  \theta  = dt H + d\x \cdot \P,
\end{equation}
so the vielbein is $E_H = \xi_{H}$ and $E_{P_a} = \xi_{P_a}$.  The
connection one-form vanishes, so it is flat, but in this case also
torsionless.  There are no other invariant affine connections.

\subsection{Homogeneous spacetime P\#9}
\label{sec:homog-spac-p9}

With $A = t H + \x \cdot \P$, we find that
\begin{equation}
  \ad_A P_a = \ad_A H = 0, \qquad \ad_A B_a = -x_a H \qquad\text{and}\qquad \ad_A Z = - \x \cdot \B,
\end{equation}
so that $\ad_A^2 Z = x^2H$ and $\ad_A^3 = 0$.  The fundamental vector
fields are found to be
\begin{equation}
  \xi_H = \frac{\d}{\d t}, \qquad \xi_Z = \tfrac12 x^2\frac{\d}{\d t},
  \qquad \xi_{B_a} = x^a \frac{\d}{\d t} \qquad\text{and}\qquad
  \xi_{P_a} = \frac{\d}{\d x^a},
\end{equation}
which indeed obey the opposite Lie algebra.

Since $\ad_A H = \ad_A P_a = 0$, we have that the soldering form is
given by
\begin{equation}
  \theta  = dt \Hbar + d\x \cdot \Pbar,
\end{equation}
so the vielbein is $E_{\Hbar} = \xi_H$ and $E_{\overline{P}_a} =
\xi_{P_a}$.  The invariant carrollian structure is given by $\xi =
\xi_H$ and $b = dx^a dx^a$.

This homogeneous spacetime admits no invariant connections.  Indeed,
if $\Lambda : \g \to \gl(\g/\h)$ is an invariant connection, then for
all $X,Y \in \g$, we have
\begin{equation}
  0 \stackrel{?}{=} \lambda_Z \Lambda_X \overline{Y} - \Lambda_X \lambda_Z
  \overline{Y} - \Lambda_{[Z,X]} \overline{Y}.
\end{equation}
But $Z$ is in the kernel of the linear isotropy representation, so
$\lambda_Z =0$ and hence only the last term survives.  Taking $X =
P_a$, this becomes
\begin{equation}
  0 \stackrel{?}{=} \Lambda_{[Z,P_a]} \overline{Y} = \Lambda_{B_a} \overline{Y} =
  \lambda_{B_a} \overline{Y},
\end{equation}
which fails for $Y=P_b$, say.

\subsection{Homogeneous spacetime P\#11}
\label{sec:homog-spac-p11}

Here we find
\begin{equation}
  \ad_A H  = 0 \qquad \ad_A \P = 0 \qquad \ad_A Z = \x \cdot \P
  \qquad\text{and}\qquad \ad_A B_a = - x_a Z - x^b J_{ab},
\end{equation}
so that
\begin{equation}
  \ad_A^2 B_a = x^2 P_a - 2 x_a \x \cdot \P
\end{equation}
and $\ad_A^3 \equiv 0$.  The fundamental vector fields are found to be
\begin{equation}
  \xi_{H} = \frac{\d}{\d t} \qquad \xi_{P_a} = \frac{\d}{\d x^a}
  \qquad \xi_Z = - x^a \frac{\d}{\d x^a} \qquad\text{and}\qquad
  \xi_{B_a} = \tfrac12 x^2 \frac{\d}{\d x^a} - x^a x^b \frac{\d}{\d x^b}.
\end{equation}
One checks that $[\xi_Z,\xi_{B_a}] = - \xi_{B_a}$, $[\xi_Z,\xi_{P_a}]
= \xi_{P_a}$ and that $[\xi_{B_a}, \xi_{P_b}] = - \delta_{ab} \xi_Z -
\xi_{J_{ab}}$, as expected.

The soldering form is given by
\begin{equation}
  \theta = dt H + d\x \cdot \P
\end{equation}
so that the vielbein is $E_{\Hbar} = \xi_{H}$ and $E_{\overline{P}_a} = \xi_{P_a}$.

This cases is non-reductive, so there is no canonical connection and,
moreover, there are no invariant affine connections.  If $\Lambda : \g
\to \gl(\g/\h)$ defines an invariant affine connection, then the
following must hold:
\begin{equation}
  0 = \lambda_{B_a} \Lambda_{P_b} \overline{P}_c - \Lambda_{[B_a,P_b]} \overline{P}_c -
  \Lambda_{P_b} \lambda_{B_a} \overline{P}_c,
\end{equation}
but we now use that $B_a$ lies in the kernel of the linear isotropy
representation\footnote{The boosts are an ideal of $\h$, but not of $\g$, so
the Klein pair $(\g,\h)$ is still effective even when the linear
isotropy representation is not faithful.} so that only the middle term
survives:
\begin{equation}
  \Lambda_{[B_a,P_b]} \overline{P}_c = \delta_{ab} \lambda_{Z} \overline{P}_c + \lambda_{J_{ab}} \overline{P}_c = -
  \delta_{ab} \overline{P}_c + \delta_{bc} \overline{P}_a - \delta_{ac} \overline{P}_b \neq 0.
\end{equation}

\subsection{Homogeneous spacetime P\#12}
\label{sec:homog-spac-p12}

Here we have that $\ad_A H = \ad_A \P = 0$, so that
\begin{equation}
  \xi_H = \frac{\d}{\d t} \qquad\text{and}\qquad \xi_{P_a} =
  \frac{\d}{\d x^a}.
\end{equation}
In addition, we have that $\ad_A Z = \x \cdot \P$ and that
\begin{equation}
  \ad_A B_a = -x^a(Z-H) - J_{ab} x^b
  \qquad \ad_A J_{ab} = x^a P_b - x^b P_a \qquad\text{and}\qquad
  \ad_A^2 B_a = x^2 P_a - 2 x^a \x \cdot \P,
\end{equation}
with $\ad_A^3 \equiv 0$.  Solving for the other fundamental vector
fields we find that
\begin{equation}
  \xi_Z = - x^a \frac{\d}{\d x^a} \qquad\text{and}\qquad \xi_{B_a} =
  \tfrac12 x^2 \frac{\d}{\d x^a} - x^a x^b \frac{\d}{\d x^b} - x^a
  \frac{\d}{\d t}.
\end{equation}
One checks that, as expected, $[\xi_Z,\xi_{B_a}] = - \xi_{B_a}$, $[\xi_Z,\xi_{P_a}]
= \xi_{P_a}$ and $[\xi_{B_a}, \xi_{P_b}] = - \delta_{ab} (\xi_Z -
\xi_H) - \xi_{J_{ab}}$.

The soldering form is given by
\begin{equation}
  \theta = dt H + d\x \cdot \P
\end{equation}
with corresponding vielbein $E_{\Hbar} = \xi_H$ and
$E_{\overline{P}_a} = \xi_{P_a}$.

Since this case is not reductive, there is no canonical invariant
connection and, indeed, there are no invariant affine connections by a
very similar argument to the one in the previous case.


\subsection{Homogeneous spacetime P\#19}
\label{sec:homog-spac-p19}

\FIXMEJ{This has to be redone since there was an error in the Lie brackets in Table~\ref{tab:gbs-effective-lie-pairs}.}

With $A = t H + \x \cdot \P$, we have that $\ad_A H = 0$, $\ad_A B_a =
- x_a H$, $\ad_A Z = -\varepsilon  \x \cdot \B$, $\ad^2_A Z =
\varepsilon x^2 H$, from where we see that
\begin{equation}
  \xi_H = \frac{\d}{\d t}, \qquad \xi_Z = \tfrac12 \varepsilon x^2
  \frac{\d}{\d t}\qquad\text{and}\qquad \xi_{B_a} = x^a \frac{\d}{\d t}.
\end{equation}

In addition, we have
\begin{equation}
  \begin{aligned}
    \ad_A P_a &= -\varepsilon x^b J_{ab}\\
    \ad^2_A P_a &= \varepsilon (x^2 P_a - x_a \x \cdot \P)\\
  \end{aligned}
  \qquad\qquad
  \begin{aligned}
    \ad_A J_{ab} &= x_a P_b - x_b P_a\\
    \ad^2_A J_{ab} &= -\varepsilon x^c (x_a J_{bc} - x_b J_{ac})\\    
  \end{aligned}
\end{equation}
and hence on the span of $\P,\J$, we have that $\ad^3_A = \varepsilon
x^2 \ad_A$.

Now, if $f(z)$ is analytic in $z$ and admits a power series expansion
$f(z) = \sum_{n=0}^\infty c_n z^n$, then
\begin{equation}
  f(\ad_A) = f(0) + \sum_{k=0}^\infty c_{2k+1} (\varepsilon x^2)^k
  \ad_A + \sum_{k=1}^\infty c_{2k} (\varepsilon x^2)^{k-1} \ad_A^2.
\end{equation}
If we let $x_\pm$ denote the two complex square roots of $\varepsilon
x^2$, with $x_- = - x_+$, then
\begin{equation}
  f(\ad_A) = f(0) + \frac1{x_+} \sum_{k=0}^\infty c_{2k+1} x_+^{2k+1}
  \ad_A + \frac1{x_+^2} \sum_{k=1}^\infty c_{2k} x_+^{2k} \ad_A^2.
\end{equation}
Observing that
\begin{equation}
  \sum_{k=0}^\infty c_{2k+1} x_+^{2k+1} = \tfrac12 ( f(x_+) - f(x_-) )
  \qquad\text{and}\qquad
  \sum_{k=1}^\infty c_{2k} x_+^{2k} = \tfrac12 ( f(x_+) + f(x_-) -
  2 f(0) ),
\end{equation}
we arrive finally at
\begin{equation}
  \label{eq:fad}
  f(\ad_A) =f(0) + \frac1{2x_+} (f(x_+)-f(x_-)) \ad_A +
  \frac{\varepsilon}{2x^2} (f(x_+) + f(x_-) - 2 f(0)) \ad_A^2.
\end{equation}

For $f(z)$ is analytic in $z$, let us introduce the shorthand notation:
\begin{equation}\label{eq:shorthand}
  f^+ := \tfrac12 (f(x_+) + f(x_-))\qquad\text{and}\qquad
  f^- := \frac1{2x_+}(f(x_+) - f(x_-)).
\end{equation}
Notice that both $f^\pm$ are invariant under the interchange of $x_+$
and $x_-$, reflecting the independence on the choice of root $x_+$.
In this shorthand notation, equation~\eqref{eq:fad} becomes
\begin{equation}
  f(\ad_A) =f(0) + f^- \ad_A + \frac{\varepsilon}{x^2} (f^+ - f(0))
  \ad_A^2.
\end{equation}

Applying this to $P_a$, we find
\begin{equation}
  f(\ad_A) P_a = f^+ P_a - \varepsilon f^- x^b J_{ab} -
  (f^+-f(0))\frac{x_a \x \cdot \P}{x^2},
\end{equation}
and hence
\begin{equation}
  f(\ad_A) J_{ab} = f(0) J_{ab} + \widetilde{f}(\ad_A) (x_a P_b - x_b P_a),
\end{equation}
where $\widetilde f(z) := (f(z)-f(0))/z$.

We now apply these formulae to calculate $\xi_{P_a}$ via
\begin{equation}
  \tau H + \y \cdot \P = G(\ad_A) \v \cdot \P - \tfrac12 \lambda^{ab} F(\ad_A) J_{ab}.
\end{equation}
One immediately sees that $\tau = 0$ and the rest expands to
\begin{equation}
  \y \cdot \P = G^+ \v \cdot \P + (1-G^+)\frac{\x\cdot\v \x \cdot
    \P}{x^2} - \lambda^{ab} \widetilde{F}^+ x_a P_b 
  - \tfrac12 \lambda^{ab} J_{ab} - \varepsilon G^- v^a x^b J_{ab} +
  \varepsilon \widetilde{F}^- \lambda^{ab} x_a x^c J_{bc}.
\end{equation}
Solving for $\lambda^{ab}$ we find
\begin{equation}
  \lambda^{ab} = \frac{\varepsilon G^-}{1+\varepsilon x^2
    \widetilde{F}^-}(x^a v^b - x^b v^a)
\end{equation}
and hence
\begin{equation}
  y^a = \left( G^+ - \frac{\varepsilon x^2 \widetilde{F}^+ G^-}{1 +
      \varepsilon x^2 \widetilde{F}^-}\right) v^a +
  \left(\frac{1-G^+}{x^2} + \frac{\varepsilon \widetilde{F}^+ G^-}{1 +
      \varepsilon x^2 \widetilde{F}^-}\right) \x \cdot \v x^a.
\end{equation}
Using the definitions of the functions $F$ and $G$, we arrive at
\begin{equation}
  y^a =
  \begin{cases}
    |\x| \coth|\x| v^a + \frac{1-|\x|\coth|\x|}{x^2} \x \cdot \v x^a & \varepsilon=1\\
    |\x| \cot|\x| v^a + \frac{1-|\x|\cot|\x|}{x^2} \x \cdot \v x^a & \varepsilon=-1,
  \end{cases}
\end{equation}
and, in summary, we find
\begin{equation}
  \begin{split}
    \xi_{P_a}^{(\varepsilon=1)} &= |\x| \coth|\x| \frac{\d}{\d x^a} +
    \frac{1-|\x|\coth|\x|}{x^2} x^a x^b \frac{\d}{\d x^b}\\
    \xi_{P_a}^{(\varepsilon=-1)}&= |\x| \cot|\x| \frac{\d}{\d x^a} +
    \frac{1-|\x|\cot|\x|}{x^2} x^a x^b \frac{\d}{\d x^b}.
  \end{split}
\end{equation}
One checks that, as expected, $[\xi_{B_a},\xi_{P_b}] = - \delta_{ab} \xi_{H}$, $[\xi_Z,\xi_{P_a}]
= -\varepsilon \xi_{B_a}$ and $[\xi_{P_a}, \xi_{P_b}] = - \varepsilon \xi_{J_{ab}}$.

The soldering form can be calculated in the same way and we arrive at
\begin{equation}
  \begin{split}
    \theta^{(\varepsilon=1)} &= dt \Hbar + \frac{\sinh|\x|}{|\x|} d\x
    \cdot \Pbar + \left( 1-\frac{\sinh|\x|}{|\x|} \right) \frac{\x\cdot
      d\x}{x^2} \x \cdot \Pbar\\
    \theta^{(\varepsilon=-1)} &= dt \Hbar + \frac{\sin|\x|}{|\x|} d\x
    \cdot \Pbar + \left( 1-\frac{\sin|\x|}{|\x|} \right) \frac{\x\cdot
      d\x}{x^2} \x \cdot \Pbar.
  \end{split}
\end{equation}
Then $\theta^{\Hbar} = dt$ in both cases and
\begin{equation}
  \theta^{\overline{P}_a}_b = s \delta^a_b + (1-s) \Pi^a_b
  \qquad\text{where}\qquad s :=
  \begin{cases}
    \frac{\sinh|x|}{|x|} & \varepsilon=1\\
    \frac{\sin|x|}{|x|} & \varepsilon=-1,
  \end{cases}
\end{equation}
and $\Pi$ is the projector $\frac{\x \x^T}{x^2}$ in matrix form.  It
is easy to invert this expression (in the unital associative algebra
generated by $\Pi$) to arrive at the vielbein
\begin{equation}
  E_{\Hbar} = \frac{\d}{\d t} \qquad\text{and}\qquad
  \begin{aligned}
    E^{(\varepsilon=1)}_{\overline{P}_a} &= |\x|\csch|\x| \frac{\d}{\d x^a} + \left(1 - |\x|\csch|\x| \right)
    \frac{x^ax^b}{x^2} \frac{\d}{\d x^b}\\
    E^{(\varepsilon=-1)}_{\overline{P}_a} &=  |\x|\csc|\x| \frac{\d}{\d x^a} + \left(1 - |\x|\csc|\x| \right)
    \frac{x^ax^b}{x^2} \frac{\d}{\d x^b}.
  \end{aligned}
\end{equation}
The invariant carrollian structure is given by $\xi = \frac{\d}{\d t}$
and
\begin{equation}
  \begin{split}
    b^{(\varepsilon=1)} &= \frac{\sinh^2|\x|}{x^2} dx^a dx^a + \left(
      1 - \frac{\sinh^2|\x|}{x^2} \right) \frac{(\x \cdot
      d\x)^2}{x^2}\\
    b^{(\varepsilon=-1)} &= \frac{\sin^2|\x|}{x^2} dx^a dx^a + \left(
      1 - \frac{\sin^2|\x|}{x^2} \right) \frac{(\x \cdot
      d\x)^2}{x^2}.   
  \end{split}
\end{equation}

Since this case is not reductive, there is no canonical invariant
connection and, indeed, there are no invariant connections.  The proof
is almost identical to that for P\#9.

\subsection{Homogeneous spacetime P\#21}
\label{sec:homog-spac-p21}

Here we have that $\ad_A H = \ad_A P = 0$, so that
\begin{equation}
  \xi_H = \frac{\d}{\d t} \qquad\text{and}\qquad \xi_{B_a} =
  \frac{\d}{\d x^a}.
\end{equation}
In addition, $\ad_A Z = -2 t H - \x \cdot \P$ and $\ad_A B_a = - x_a
H$, with $\ad_A^2 \equiv 0$.  Solving for the fundamental vector
fields, we find
\begin{equation}
  \xi_Z = 2 t \frac{\d}{\d t} + x^a\frac{\d}{\d x^a}
  \qquad\text{and}\qquad
  \xi_{B_a} = x^a \frac{\d}{\d t}.
\end{equation}
One checks that the Lie brackets of the fundamental vector fields are
as expected.

The soldering form is again
\begin{equation}
  \theta = dt H +  d\x \cdot \P
\end{equation}
with vielbein $E_H = \frac{\d}{\d t}$ and $E_{P_a} = \frac{\d}{\d x^a}$.

The connection one-form vanishes and the canonical connection is not
just flat but also torsion-free.  There is a one-parameter family of
invariant connections characterised by the Nomizu map
\begin{equation}
  \alpha(P_a, P_b) = \mu \delta_{ab} H.
\end{equation}
All invariant connections are flat and torsion-free.

\subsection{Homogeneous spacetimes P\#23 and P\#25}
\label{sec:homog-spac-p23-25}

We may treat these two cases together by considering $[\B,\P] = H$,
$[Z,\B] = \beta \P$, $[Z,\P] = \pi \P$ and $[Z,H] = (\beta + \pi) H$,
where $\beta + \pi = 1+ \gamma \in (0,2)$.  For P\#23$_\gamma$,
$(\beta,\pi) = (\gamma, 1)$, whereas for P\#25$_\gamma$, $(\beta,\pi)
= (1,\gamma)$.

Since $\ad_A H = \ad_A \P = 0$, we have that
\begin{equation}
  \xi_H = \frac{\d}{\d t} \qquad\text{and}\qquad \xi_{P_a} =
  \frac{\d}{\d x^a}.
\end{equation}
On the other generators,
\begin{equation}
  \ad_A Z = - (1+\gamma) H - \pi \x \cdot \P \qquad\text{and}\qquad
  \ad_A \B = - \x H,
\end{equation}
so that $\ad_A^2 \equiv 0$.  Solving for the other fundamental vector
fields, we find
\begin{equation}
  \xi_Z = (1+\gamma) \frac{\d}{\d t} + \pi x^a \frac{\d}{\d x^a}
  \qquad\text{and}\qquad
  \xi_{B_a} = x^a \frac{\d}{\d t}.
\end{equation}

The soldering form and vielbein are
\begin{equation}
  \theta = dt H + d\x \cdot \P \implies E_H = \xi_H
  \quad\text{and}\quad E_{P_a} = \xi_{P_a}.
\end{equation}
The connection one-form vanishes, so that the canonical connection is
flat and also torsion-free.  The canonical connection is the unique
invariant affine connection on these homogeneous spacetimes.

\subsection{Homogeneous spacetime P\#28}
\label{sec:homog-spac-p28}

Here $\ad_A H = \ad_A \P = 0$, so that
\begin{equation}
  \xi_H = \frac{\d}{\d t} \qquad\text{and}\qquad
  \xi_{P_a} = \frac{\d}{\d x^a}.
\end{equation}
On other generators we have that
\begin{equation}
  \ad_A Z = -2 t H - \x \cdot \P - \x \cdot \B, \qquad \ad_A^2 Z = x^2
  H \qquad\text{and}\qquad \ad_A \B = -\x H,
\end{equation}
with $\ad_A^3 \equiv 0$.  Solving for the remaining fundamental vector
fields, we find
\begin{equation}
  \xi_Z = (2t + \tfrac12 x^2) \frac{\d}{\d t} + x^a \frac{\d}{\d x^a}
  \qquad\text{and}\qquad
  \xi_{B_a} = x^a \frac{\d}{\d t}.
\end{equation}
We check that their Lie brackets are as expected.

The soldering form and vielbein are given by
\begin{equation}
  \theta = dt H + d\x \cdot \P \implies E_H = \frac{\d}{\d t}
  \quad\text{and}\quad E_{P_a} = \frac{\d}{\d x^a}.
\end{equation}
This is a non-reductive example, so there is no canonical connection
and, indeed, there is no invariant connection.  This follows most
easily by demanding that $\Lambda_{P_a} P_b$ is invariant under $Z$,
which yields a contradiction.

\subsection{Homogeneous spacetime P\#31}
\label{sec:homog-spac-p31}

Here we have $\ad_A H = \ad_A P_a = 0$, so that again
\begin{equation}
  \xi_H = \frac{\d}{\d t} \qquad\text{and}\qquad
  \xi_{P_a} = \frac{\d}{\d x^a}.
\end{equation}
On the other generators, $\ad_A^2 \equiv 0$ and
\begin{equation}
  \ad_A Z = -t H - \x \cdot \P \qquad\text{and}\qquad \ad_A \B = 
  \varepsilon t \P - \x H.
\end{equation}
We solve for the fundamental vector fields and obtain
\begin{equation}
  \xi_Z = t \frac{\d}{\d t} + x^a \frac{\d}{\d x^a}
  \qquad\text{and}\qquad
  \xi_{B_a} = x^a \frac{\d}{\d t} - \varepsilon t \frac{\d}{\d x^a}.
\end{equation}
One checks that their Lie brackets are as expected.

The soldering form and the vielbein are given by
\begin{equation}
  \theta = dt H + d\x \cdot \P \implies E_H = \frac{\d}{\d t}
  \quad\text{and}\quad E_{P_a} = \frac{\d}{\d x^a}.
\end{equation}
The connection one-form vanishes, showing that the canonical
connection is flat.  It is also torsion-free.  Moreover, invariance
under $Z$ already shows that there are no nonzero Nomizu maps, so that
the canonical connection is the unique invariant affine connection
here.

\subsection{Homogeneous spacetime P\#33}
\label{sec:homog-spac-p33}

In this case, $[\B,\P] = H$, so that $\B$ acts via
``carrollian boosts'' and hence we can immediately write down
\begin{equation}
  \xi_{B_a} = x^a \frac{\d}{\d t},
\end{equation}
whereas $Z$ grades the algebra with $H$ having weight $1$ and $\P$
weight zero, so
\begin{equation}
  \xi_{Z} = t \frac{\d}{\d t}.
\end{equation}
One checks that indeed $[\xi_Z, \xi_{B_a}] = - \xi_{B_a}$, as
expected.

The adjoint action of $A = tH + \x \cdot \P$ is given by
\begin{equation}
  \begin{split}
    \ad_A H &= \varepsilon \x \cdot \B\\
    \ad_A Z &= -t H\\
    \ad_A B_a &= - x^a H\\
    \ad_A P_a &= -\varepsilon t B_a - \varepsilon x^b J_{ba}\\
    \ad_A J_{ab} &=x^a P_b - x^b P_a.
  \end{split}
\end{equation}
Iterating we find that
\begin{equation}
  \begin{split}
    \ad^2_A H &= -\varepsilon x^2 H\\
    \ad^2_A Z &= - \varepsilon t \x \cdot \B\\
    \ad^2_A B_a &= - \varepsilon x^a \x \cdot \B \\
    \ad^2_A P_a &=\varepsilon t x^a H + \varepsilon x^a \x \cdot \P -
    \varepsilon x^2 P_a\\
    \ad^2_A J_{ab} &= - \varepsilon t (x_a B_b - x_b B_a) -
    \varepsilon x^c (x_a J_{cb} - x_b J_{ca}),
  \end{split}
\end{equation}
and further that $\ad_A^3 = -\varepsilon x^2 \ad_A$.  As we did in the
case of P\#19, we arrive at the formula:
\begin{equation}
  f(\ad_A) =f(0) + f^- \ad_A - \frac{\varepsilon}{x^2} (f^+ - f(0)) \ad_A^2,
\end{equation}
where $f^\pm$ are given by equation~\eqref{eq:shorthand}, with $x_\pm$
the two (complex) square roots of $-\varepsilon x^2$ with $x_- = - x_+$.

Applying this to the basis,
\begin{equation}
  \begin{split}
    f(\ad_A) H &= f^+ H + \varepsilon f^- \x \cdot \B\\
    f(\ad_A) Z &= f(0) Z - t f^- H +  \frac{t}{x^2} (f^+ - f(0)) \x \cdot \B\\
    f(\ad_A) B_a &= f(0) B_a - x^a f^- H + \frac{x^a}{x^2} (f^+ - f(0)) \x \cdot \B \\
    f(\ad_A) P_a &= f^+ P_a + \varepsilon f^- (x^b J_{ab} - t B_a) - \frac{x^a}{x^2}(f^+ - f(0))(tH + \x\cdot \P) \\
  \end{split}
\end{equation}
and hence on $J_{ab}$,
\begin{equation}
  f(\ad_A) J_{ab} = f(0) J_{ab} + x^a \widetilde{f}(\ad_A) P_b - x^b \widetilde{f}(\ad_A) P_a,
\end{equation}
where $\widetilde{f}(z)= (f(z)-f(0))/z$.

We now apply these formulae in order to solve for $\xi_H$ and $\xi_{P_a}$.
To find $\xi_H$, we solve
\begin{equation}
  \tau H + \y \cdot \P = G(\ad_A) H - F(\ad_A) \w \cdot \B
\end{equation}
for $\tau$, $\y$ and $\w$, which results in
\begin{equation}
  \w = \frac{\varepsilon G^-}{F^+} \x,
\end{equation}
and hence $\y = 0$ and
\begin{equation}
  \tau = \frac{G(t_+)F(t_-) + G(t_-) F(t_+)}{F(x_+)+F(x_-)} =
  \begin{cases}
    |\x| \cot|\x| & \varepsilon=+1\\
    |\x| \coth|\x| & \varepsilon=-1.
  \end{cases}
\end{equation}
Therefore,
\begin{equation}
  \xi^{(\varepsilon=1)}_H = |\x| \cot|\x| \frac{\d}{\d t}
  \qquad\text{and}\qquad
  \xi^{(\varepsilon=-1)}_H = |\x| \coth|\x| \frac{\d}{\d t}.
\end{equation}

To find $\xi_{P_a}$ we solve
\begin{equation}
  \tau H + \y \cdot \P = G(\ad_A) \v\cdot \P - F(\ad_A) \left(\w \cdot \B -
  \tfrac12 \lambda^{ab} J_{ab}\right)
\end{equation}
for $\tau$, $\y$, $\w$ and $\lambda^{ab}$.  The $J_{ab}$ terms give
the equation
\begin{equation}
  \label{eq:lambda}
  \lambda^{ab} = \varepsilon G^- (v^a x^b - v^b x^a) - \varepsilon
  \widetilde{F}^- (\lambda^{bc} x^c x^a - \lambda^{ac} x^c x^b).
\end{equation}
Contracting with $x^b$ we find
\begin{equation}
  \lambda^{ab} x^b = \frac{\varepsilon G^- (x^2 v^a - \x\cdot \v
    x^a)}{1-\varepsilon x^2 \widetilde{F}^-},
\end{equation}
and plugging it back into equation~\eqref{eq:lambda}, we find
\begin{equation}
  \lambda^{ab} = \frac{\varepsilon G^-}{1-\varepsilon x^2
    \widetilde{F}^-} (v^a x^b - v^b x^a).
\end{equation}
The $\B$ terms give the following equation
\begin{equation}
  \label{eq:w}
  w^a = - \varepsilon t G^- v^a - \frac{(F^+-1)\x\cdot\w x^a}{x^2} -
  \frac{\widetilde{F}^-G^- t}{1-\varepsilon x^2 \widetilde{F}^-} (x^2
  v^a - \x \cdot \v x^a).
\end{equation}
Contracting with $x^a$, we find
\begin{equation}
  \w \cdot \x = \frac{-\varepsilon G^- t}{F^+} \x \cdot \v,
\end{equation}
and plugging back into equation \eqref{eq:w} gives us
\begin{equation}
  w^a = \left(\frac{\varepsilon t G^-}{x^2} + \frac{\widetilde{F}^-
      G^- t}{1-\varepsilon x^2 \widetilde{F}^-}\right) (\x \cdot \v
  x^a - x^2 v^a) - \frac{\varepsilon t G^-}{x^2 F^+} \x \cdot \v x^a.
\end{equation}
The $H$ terms give
\begin{equation}
  \tau = - t \x \cdot \v \left(\frac{G^+-1}{x^2} + \frac{\varepsilon
      F^- G^-}{F^+}\right) =
  \begin{cases}
    \frac{t}{x^2} (1 - |\x|\cot|\x|) \x \cdot \v& \varepsilon=1\\
    \frac{t}{x^2} (1 - |\x|\coth|\x|) \x \cdot \v & \varepsilon=-1.
  \end{cases}
\end{equation}
Finally, the $\P$ terms give
\begin{equation}
  y^a = \left(G^+ + \frac{\varepsilon G^- \widetilde{F}^+
      x^2}{1-\varepsilon x^2 \widetilde{F}^-}\right) v^a - \left(
    \frac{G^+-1}{x^2} + \frac{\varepsilon
      G^-\widetilde{F}^+}{1-\varepsilon x^2 \widetilde{F}^-}\right) \x
  \cdot \v x^a
\end{equation}
which simplifies to
\begin{equation}
  y^a =
  \begin{cases}
    |\x| \cot|\x| v^a + \frac{1-|\x|\cot|\x|}{x^2} \x \cdot \v x^a & \varepsilon=1\\
    |\x| \coth|\x| v^a + \frac{1-|\x|\coth|\x|}{x^2} \x \cdot \v x^a & \varepsilon=-1.
  \end{cases}
\end{equation}
In summary, we find
\begin{equation}
  \begin{split}
    \xi_{P_a}^{(\varepsilon=1)}&= \frac{t}{x^2} (1 - |\x|\cot|\x|)
    x^a \frac{\d}{\d t} + |\x| \cot|\x| \frac{\d}{\d x^a} +
    \frac{1-|\x|\cot|\x|}{x^2} x^a x^b \frac{\d}{\d x^b}\\
    \xi_{P_a}^{(\varepsilon=-1)} &= \frac{t}{x^2} (1 - |\x|\coth|\x|)
    x^a \frac{\d}{\d t} + |\x| \coth|\x| \frac{\d}{\d x^a} +
    \frac{1-|\x|\coth|\x|}{x^2} x^a x^b \frac{\d}{\d x^b}.
  \end{split}
\end{equation}
One checks that, for $\varepsilon=1$ and $\varepsilon=-1$, we get 
$[\xi_{B_a},\xi_{P_b}] = - \delta_{ab} \xi_{H}$, $[\xi_Z,\xi_{B_a}]
= - \xi_{B_a}$, $[\xi_{H},\xi_{P_a}] = \varepsilon \xi_{B_a}$, 
$[\xi_{Z},\xi_{H}] = - \xi_{H}$ and $[\xi_{P_a}, \xi_{P_b}] = \varepsilon \xi_{J_{ab}}$.

The soldering form is given by
\begin{equation}
  \begin{split}
    \theta^{(\varepsilon=1)} &= \frac{\sin|\x|}{|\x|} (dt H + d\x
    \cdot \P) + \left( 1-\frac{\sin|\x|}{|\x|} \right) \frac{\x\cdot
      d\x}{x^2} (t H + \x\cdot \P)\\
    \theta^{(\varepsilon=-1)} &= \frac{\sinh|\x|}{|\x|} (dt H + d\x
    \cdot \P) + \left( 1-\frac{\sinh|\x|}{|\x|} \right) \frac{\x\cdot
      d\x}{x^2} (t H + \x\cdot \P)
  \end{split}
\end{equation}
and the connection one-form of the canonical connection is given by
\begin{equation}
  \begin{split}
    \omega^{(\varepsilon=1)} &= \frac{\cos|\x|}{x^2} \left(dt \x \cdot \B -
    t d\x \cdot \B + dx^a x^b J_{ab}\right)\\
    \omega^{(\varepsilon=-1)} &= \frac{\cosh|\x|}{x^2} \left(dt \x \cdot \B -
    t d\x \cdot \B + dx^a x^b J_{ab}\right).
  \end{split}
\end{equation}
Being symmetric, the canonical connection is torsion-free, but it is
not flat:
\begin{equation}
  \begin{split}
    \Omega^{(\varepsilon=1)} &= \frac{\sin^2|\x|}{x^2}dx^a \wedge dx^b
    J_{ab} + \frac{\sin|\x|}{|\x|} \left( 1 - \frac{\sin|\x|}{|\x|}
    \right) \frac{x^b x^c}{x^2} (dx^a \wedge dx^c J_{ab} + dt \wedge
    dx^c B_b)\\
    \Omega^{(\varepsilon=-1)} &= \frac{\sinh^2|\x|}{x^2}dx^a \wedge dx^b
    J_{ab} + \frac{\sinh|\x|}{|\x|} \left( 1 - \frac{\sinh|\x|}{|\x|}
    \right) \frac{x^b x^c}{x^2} (dx^a \wedge dx^c J_{ab} + dt \wedge
    dx^c B_b).
  \end{split}
\end{equation}

The vielbein inverse to the soldering form is given by
\begin{equation}
  \begin{split}
    E_H^{(\varepsilon=1)} &= |\x|\csc|\x| \frac{\d}{\d t}\\
    E_{P_a}^{(\varepsilon=1)} &= |\x|\csc|\x| \frac{\d}{\d x^a} + (1 -
    |\x|\csc|\x|) \frac{x^a}{x^2} \left(t \frac{\d}{\d t} + x^b
      \frac{\d}{\d x^b}\right)
  \end{split}
\end{equation}
and
\begin{equation}
  \begin{split}
    E_H^{(\varepsilon=-1)} &= |\x|\csch|\x| \frac{\d}{\d t}\\
    E_{P_a}^{(\varepsilon=-1)} &= |\x|\csch|\x| \frac{\d}{\d x^a} + (1 -
    |\x|\csch|\x|) \frac{x^a}{x^2} \left(t \frac{\d}{\d t} + x^b
      \frac{\d}{\d x^b}\right).
  \end{split}
\end{equation}


The canonical connection is the unique invariant connection:
invariance under rotations and under $Z$, which gives weight $1$ to
$H$ but $0$ to $\P$, kills every component of the Nomizu map except
possibly $\alpha(P_a,P_b)$ (and even then only in $D=3$), but then
invariance under $\B$ kills that component as well.




==> Generalised_Bargmann_Spacetimes/Intro/intro.tex <==
intro

==> Generalised_Bargmann_Spacetimes/main.tex <==
% This is just a super-short file to collect all the sections of the non-SUSY 
% Bargmann section together in one place. 
\input{Generalised_Bargmann_Spacetimes/Intro/intro}

\section{Classification of Generalised Bargmann Algebras}
\input{Generalised_Bargmann_Spacetimes/GBAs/gba}

\section{Classification of Bargmann Spacetimes and Homogeneous Bargmann Spaces}
\input{Generalised_Bargmann_Spacetimes/GBSs/gbs}

\section{Geometric Properties of Bargmann Spacetimes and Homogeneous Bargmann Spaces}
\input{Generalised_Bargmann_Spacetimes/GPs/gps}

==> Mathematical_Preliminaries/Geometric_Properties/KSS/kss.tex <==
kss
